Is Temporal Difference Learning Optimal? An Instance-Dependent Analysis

We address the problem of policy evaluation in discounted Markov decision processes, and provide instance-dependent guarantees on the $\ell_\infty$-error under a generative model. We establish both asymptotic and non-asymptotic versions of local minimax lower bounds for policy evaluation, thereby providing an instance-dependent baseline by which to compare algorithms. Theory-inspired simulations show that the widely-used temporal difference (TD) algorithm is strictly suboptimal when evaluated in a non-asymptotic setting, even when combined with Polyak-Ruppert iterate averaging. We remedy this issue by introducing and analyzing variance-reduced forms of stochastic approximation, showing that they achieve non-asymptotic, instance-dependent optimality up to logarithmic factors.

==> DinosaurMacros-arXiv <==

\newcommand{\LOGDN}{\ensuremath{\sqrt{\LOGDNSQ}}}
\newcommand{\LOGDNSQ}{\ensuremath{\frac{\log(8 \Dim/\delta)}{\Nsamp}}}

\newcommand{\sighat}{\ensuremath{\widehat{\sigma}}}
\newcommand{\IdMat}{\ensuremath{\mathbf{I}}}
\newcommand{\Phat}{\ensuremath{\widehat{\Pmat}}}

\newcommand{\Ptranshat}{\ensuremath{\widehat{P}}}

\newcommand{\Enoise}{\ensuremath{W}}

\newcommand{\thetaopt}{\ensuremath{\theta^*}}
\newcommand{\tddim}{\ensuremath{D}}
\newcommand{\thetapol}{\ensuremath{\theta_\pol}}
\newcommand{\futurevec}{\ensuremath{\xi}}
\newcommand{\PhiDiff}{\ensuremath{\mathbf{\Psi}}}
\newcommand{\PhiPlain}{\ensuremath{\mathbf{\Phi}}}
  
\newcommand{\thetanaive}{\ensuremath{\thetahat_{\mbox{\tiny{nai}}}}}
\newcommand{\rewardvec}{\ensuremath{r}}
\newcommand{\thetalstd}{\ensuremath{\thetahat_{\mbox{\tiny{lstd}}}}}



\newcommand{\vnoise}[1]{\ensuremath{v_{#1}}}
\newcommand{\Vnoise}{\ensuremath{W}}
\newcommand{\VnoiseIt}[1]{\ITCOMMAND{\Vnoise}{#1}}

\newcommand{\statedim}{\ensuremath{d}}
\newcommand{\condim}{\ensuremath{k}}




\renewcommand{\time}{\ensuremath{t}}
\newcommand{\xstate}[1]{\ensuremath{x_{#1}}}
\newcommand{\ystate}[1]{\ensuremath{y_{#1}}}
\newcommand{\ucon}[1]{\ensuremath{u_{#1}}}
\newcommand{\wnoise}[1]{\ensuremath{w_{#1}}}


\newcommand{\Jcost}{\ensuremath{\mathcal{J}}}

\newcommand{\UcostMat}{\ensuremath{\Rmat}}
\newcommand{\XcostMat}{\ensuremath{\Qmat}}
\newcommand{\numaction}{\ensuremath{m}}
\newcommand{\numstate}{\ensuremath{d}}
\newcommand{\NoiseCov}{\ensuremath{\Nmat}}
\newcommand{\ValMat}{\ensuremath{\Pmat}}

\newcommand{\uconstar}[1]{\ensuremath{u^*_{#1}}}
\newcommand{\ValMatStar}{\ensuremath{\ValMat^\ast}}

\newcommand{\cost}{\ensuremath{c}}
\newcommand{\Cost}{\ensuremath{\mathcal{C}}}

\newcommand{\fulltracer}[2]{\ensuremath{\trace{\big(#1 #2 \big)}}}


%\newcommand{\BellmanPolIter}[1]{\ensuremath{\Bellman_{#1}}}
\newcommand{\myoperator}[1]{\mathcal{#1}}

\newcommand{\DiffOp}{\ensuremath{\myoperator{D}}}

\newcommand{\PmatSubpol}[1]{\ensuremath{\Pmat_{#1}}}
\newcommand{\PmatPol}{\PmatSubpol{\pol}}
\newcommand{\PmatOpt}{\ensuremath{\Pmat^{*}}}

\newcommand{\rewardpol}{\ensuremath{r_\pol}}
\newcommand{\Greedy}{\ensuremath{\myoperator{G}}}

\newcommand{\statestar}{\ensuremath{\state^\dagger}}
\newcommand{\SSUM}{\ensuremath{\sum_{\nextstate \in \StateSpace}}}

\newcommand{\ValFunTil}{\ensuremath{\widetilde{\ValFun}}}
\newcommand{\ValfunTil}{\ValFunTil}
\newcommand{\Valfuntil}{\ValFunTil}
\newcommand{\poltil}{\ensuremath{\widetilde{\pol}}}
\newcommand{\ValFunPolTil}{\ensuremath{\ValFunTil^{\poltil}}}
\newcommand{\ValfunPolTil}{\ValFunPolTil}
\newcommand{\ValfunPoltil}{\ValFunPolTil}


\newcommand{\bigdim}{\ensuremath{d}}

\newcommand{\Id}{\ensuremath{\mathbf{I}}}
\newcommand{\DelPop}{\ensuremath{\mathbb{\Delta}}}
\newcommand{\DelEmp}{\ensuremath{\hat{\DelPop}}}


\newcommand{\ITER}[2]{#1_{#2}}
\newcommand{\Tepoch}{\ensuremath{K}}
\newcommand{\TepochIt}[1]{\ensuremath{\ITER{\Tepoch}{#1}}}

\newcommand{\EnoiseIter}[1]{\ITCOMMAND{\Enoise}{#1}}
\newcommand{\supperit}[1]{\ITCOMMAND{\bar{S}}{#1}}
\newcommand{\slowerit}[1]{\ensuremath{\ITCOMMAND{\underbar{\emph{S}}}{#1}}}
\newcommand{\detit}[1]{\ITCOMMAND{b}{#1}}

\newcommand{\ITCOMMAND}[2]{\ensuremath{#1}_{#2}}
\newcommand{\pathit}[1]{\ITCOMMAND{P}{#1}}
\newcommand{\pathitprime}[1]{\ITCOMMAND{P'}{#1}}
\newcommand{\pathitlower}[1]{\ITCOMMAND{\underbar{\emph{P}}}{#1}}
\newcommand{\pathitupper}[1]{\ITCOMMAND{\bar{\emph{P}}}{#1}}
\newcommand{\avarit}[1]{\ITCOMMAND{a}{#1}}
\newcommand{\avaritupper}[1]{\ITCOMMAND{\bar{A}}{#1}}
\newcommand{\avaritlower}[1]{\ITCOMMAND{\underbar{A}}{#1}}

\newcommand{\zerovec}{\ensuremath{\mathbb{0}}}
\newcommand{\onevec}{\ensuremath{\mathbf{1}}}


\newcommand{\thetait}[1]{\ITCOMMAND{\theta}{#1}}
\newcommand{\DeltaIt}[1]{\ITCOMMAND{\Delta}{#1}}
\newcommand{\DelIt}[1]{\DeltaIt{#1}}
\newcommand{\wnoiseit}[1]{\ITCOMMAND{W}{#1}}
\newcommand{\epsnoiseit}[1]{\ITCOMMAND{E}{#1}}
\newcommand{\vnoiseit}[1]{\ITCOMMAND{v}{#1}}
\newcommand{\Hop}{\ensuremath{\mathcal{H}}}
\newcommand{\HopIter}[1]{\ensuremath{\ITCOMMAND}{\Hop}{#1}}
\newcommand{\TopIter}[1]{\ensuremath{\ITCOMMAND}{\Top}{#1}}
\newcommand{\epoch}{\ensuremath{T}}
\newcommand{\epochnew}{\ensuremath{{\epoch_{+}}}}
\newcommand{\const}{\ensuremath{\nu}}
\newcommand{\titer}{\ensuremath{k}}
\newcommand{\stochit}[1]{\ITCOMMAND{#1}}
\newcommand{\Wrunit}[1]{\ITCOMMAND{W}{#1}}


\newcommand{\Pol}{\ensuremath{\Pi}}

\newcommand{\ExsOpt}{\ensuremath{\Exs^*}}
\newcommand{\ExsPol}{\ensuremath{\Exs^\pol}}

\newcommand{\state}{\ensuremath{x}}
\newcommand{\action}{\ensuremath{u}}
\newcommand{\actionopt}{\ensuremath{\action^*}}
\newcommand{\State}{\ensuremath{X}}
\newcommand{\Action}{\ensuremath{U}}
\newcommand{\reward}{\ensuremath{r}}
\newcommand{\rhat}{\ensuremath{\widehat{r}}}
\newcommand{\Reward}{\ensuremath{R}}

\newcommand{\nextstate}{\ensuremath{\state'}}
\newcommand{\Nextstate}{\ensuremath{\State'}}

\newcommand{\nextaction}{\ensuremath{\action'}}
\newcommand{\Nextaction}{\ensuremath{\Action'}}

\newcommand{\TfunPlain}{\ensuremath{\mathbb{P}}}
\newcommand{\Trans}[3]{\ensuremath{\TfunPlain_{#2}(#3 \mid #1)}}
\newcommand{\Tfun}{\Trans}
\newcommand{\TransPlain}{\TfunPlain}

\newcommand{\discount}{\ensuremath{\gamma}}

\newcommand{\Bellman}{\ensuremath{\myoperator{T}}}
\newcommand{\BellmanOpt}{\ensuremath{\Bellman^*}}
\newcommand{\BellmanPol}{\ensuremath{\Bellman_\pol}}
\newcommand{\EmpBellman}{\ensuremath{\widehat{\Bellman}}}
\newcommand{\EmpBellmanIter}[1]{\ITCOMMAND{\EmpBellman}{#1}}
\newcommand{\BellmanIter}[1]{\ITCOMMAND{\Bellman}{#1}}
	
\newcommand{\Qfun}{\ensuremath{Q}}
\newcommand{\QfunIter}[1]{\ITCOMMAND{\Qfun}{#1}}

\newcommand{\Valfun}{\ensuremath{V}}
\newcommand{\ValFun}{\ensuremath{\Valfun}}
\newcommand{\Valopt}{\ensuremath{\Valfun^*}}  
\newcommand{\ValOpt}{\ensuremath{\Valopt}}

\newcommand{\ValfunIter}[1]{\Valfun_{#1}}
\newcommand{\BellmanPolIter}[1]{\Bellman_{\pol_#1}}

\newcommand{\pol}{\ensuremath{\pi}}
\newcommand{\polhat}{\ensuremath{\widehat{\pi}}}
\newcommand{\polit}[1]{\ensuremath{\pol_{#1}}}
\newcommand{\polopt}{\ensuremath{\pol^*}}
\newcommand{\Qfunpol}{\ensuremath{\Qfun_\pol}}
\newcommand{\QfunPol}{\Qfunpol}
\newcommand{\QfunOpt}{\Qfunopt}
\newcommand{\Qfunopt}{\ensuremath{\Qfun^*}}
\newcommand{\Valfunpol}{\ensuremath{\Valfun_\pol}}
\newcommand{\ValFunPol}{\Valfunpol}
\newcommand{\Valfunopt}{\ensuremath{\Valfun^*}}
\newcommand{\ValfunPol}{\Valfunpol}
\newcommand{\ValfunOpt}{\Valfunopt}

\newcommand{\ActionSpace}{\ensuremath{\mathcal{U}}}
\newcommand{\StateSpace}{\ensuremath{\mathcal{X}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\StageCost}{\ensuremath{\psi}}

\newcommand{\iter}{\ensuremath{\ell}}
\newcommand{\xit}[1]{\ensuremath{x_{#1}}}
\newcommand{\stepit}[1]{\ensuremath{\stepcon_{#1}}}
\newcommand{\ffun}{\ensuremath{f}}
\newcommand{\Tfinal}{\ensuremath{T}}
\newcommand{\Tmax}{\Tfinal}
\newcommand{\xinit}{\ensuremath{\xit{0}}}
\newcommand{\sconvex}{\ensuremath{m}}
\newcommand{\stepcon}{\ensuremath{\lambda}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\FORALLXY}{\mbox{for all $x, y \in \real^d$}}
%\newcommand{\Constraint}{\ensuremath{\mathcal{C}}}

\newcommand{\PROJ}{\ensuremath{\Pi_\Constraint}}
\newcommand{\PROJC}{\PROJ}
\newcommand{\xstar}{\ensuremath{x^*}}
\newcommand{\GRADC}{\ensuremath{g_{\texttt{prox}}}}
%\newcommand{\myspan}{\ensuremath{\mbox{sp}}}

\newcommand{\dom}{\ensuremath{\mbox{dom}}}

\newcommand{\NormCone}{\ensuremath{\mathcal{N}}}
\newcommand{\TangCone}{\ensuremath{\mathcal{T}}}

%\newcommand{\Ind}{\ensuremath{\mathbb{I}}}

\newcommand{\distC}{\genDist{\Constraint}}
\newcommand{\genDist}[1]{\ensuremath{\mbox{dist}_{#1}}}

\newcommand{\myint}{\ensuremath{\mbox{int}}}


\newcommand{\PROX}[1]{\ensuremath{\mbox{\texttt{prox}}_{#1}}}
\newcommand{\hfun}{\ensuremath{h}}

\newcommand{\Lperp}{\ensuremath{\Lspace^\perp}}
\newcommand{\Kstar}{\ensuremath{K^*}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\newcommand{\CliqueNum}{\ensuremath{\mathcal{C}}}

\newcommand{\HANAERR}{\ensuremath{\varepsilon_\numobs}}

\newcommand{\singtrace}{\ensuremath{\operatorname{tr}}}

\newcommand{\INDSTARI}{\ensuremath{\mathbb{I}[|\inprod{\thetastar}{x_i}|
      \leq T]}}
\newcommand{\INDSTAR}{\ensuremath{\mathbb{I}[|\inprod{\thetastar}{x}|
      \leq T]}}
\newcommand{\INDSTARCOM}{\ensuremath{\mathbb{I}[|\inprod{\thetastar}{x}|
      > T]}}
\newcommand{\TRUNFUNSPEC}[1]{\ensuremath{\varphi_{\trunpar(#1)}}}

\newcommand{\trunpar}{\ensuremath{\tau}}

\newcommand{\TRUNFUNTWO}{\ensuremath{\widetilde{\varphi}_\trunpar}}

\newcommand{\Excess}{\ensuremath{E}}

\newcommand{\myparagraph}[1]{\noindent {\emph{#1}} $\;$}
\newcommand{\MYPARAGRAPH}[1]{\noindent {\emph{#1}} $\;$}

\newcommand{\realepscrit}{\ensuremath{\varepsilon_\numobs}}

\newcommand{\mccon}{\ensuremath{\beta}}

\newcommand{\NSUP}{\ensuremath{N_{\mathrm{sup}}}}

%\newcommand{\Qbar}{\ensuremath{\widebar{\qprob}}}
\newcommand{\Qbar}{\ensuremath{\bar{\qprob}}}
\newcommand{\mypackdens}[1]{\ensuremath{f_{#1}}}
\newcommand{\mypackprob}[1]{\ensuremath{\mprob_{#1}}}

\newcommand{\SetClassZero}{\ensuremath{\SetClass_0}}
\newcommand{\SetClassOne}{\ensuremath{\SetClass_1}}


\newcommand{\vcprime}[1]{\ensuremath{\vc'(#1)}}

\newcommand{\MSMALL}{\ensuremath{C}} 

\newcommand{\half}{\ensuremath{\frac{1}{2}}}

\newcommand{\KLETSET}{\ensuremath{\Ball_{2, \Phi}}}
\newcommand{\rad}{\ensuremath{\rho}}
\newcommand{\bigrad}{\ensuremath{R}}

\newcommand{\ScaleFun}{\ensuremath{\Psi}}

\newcommand{\DiagCovHat}{\ensuremath{\mathbf{\widehat{D}}}}
\newcommand{\CovMatTil}{\ensuremath{\widetilde{\CovMat}}} 




\newcommand{\fdens}{f_0}

\newcommand{\alphastar}{\ensuremath{\alpha^*}}
\newcommand{\DelHatAlpha}{\ensuremath{\DelHat_{\alpha}}}
\newcommand{\DelHatBeta}{\ensuremath{\DelHat_{\beta}}}
\newcommand{\DeltaAlpha}{\ensuremath{\Delta_{\alpha}}}
\newcommand{\DeltaBeta}{\ensuremath{\Delta_{\beta}}}

\newcommand{\mytiny}[1]{\mbox{\scalebox{.5}{#1}}}
\newcommand{\mylarge}[1]{\mbox{\scalebox{.8}{#1}}}



%\newcommand{\tmpAset}{\ensuremath{\mathbb{L}_0}}
%\newcommand{\tmpBset}{\ensuremath{\mathbb{L}_1}} 
%\newcommand{\clconv}{\ensuremath{\widebar{\mathrm{conv}}}}



\newcommand{\delmax}{\ensuremath{\delta_{\numobs, \mathrm{max}}}}

\newcommand{\FclassEllOne}{\ensuremath{\Fclass_{\ell_1}}}

\newcommand{\Jlow}{\ensuremath{\GamMat_{\mathrm{low}}}}

\newcommand{\pertvec}{\ensuremath{\Delta}}

\newcommand{\myspan}{\ensuremath{\operatorname{span}}}
\newcommand{\tagtheta}{\ensuremath{\beta}}


\newcommand{\hildist}{\ensuremath{\rho_\Hil}}


\newcommand{\SUPERSHATTER}[1]{\ensuremath{\Phi_{#1}}}
\newcommand{\UPPER}[1]{\ensuremath{\Psi_{#1}}}
\newcommand{\kindex}{\ensuremath{k}}


\newcommand{\GamMat}{\ensuremath{\mathbf{\Gamma}}}
\newcommand{\ThetaMat}{\ensuremath{\mathbf{\Theta}}}
\newcommand{\ThetaRR}{\ensuremath{\widehat{\ThetaMat}_{\mathrm{RR}}}}
\newcommand{\LamMat}{\ensuremath{\mathbf{\Lambda}}}

\newcommand{\specthetatil}{\ensuremath{\widetilde{\gamma}}}

\newcommand{\FclassAdd}{\ensuremath{\Fclass_{\mathrm{add}}}}



\newenvironment{carlist}
 {\begin{list}{$\bullet$}
 {\setlength{\topsep}{0in} \setlength{\partopsep}{0in}
  \setlength{\parsep}{0in} \setlength{\itemsep}{\parskip}
  \setlength{\leftmargin}{0.15in} \setlength{\rightmargin}{0.08in}
  \setlength{\listparindent}{0in} \setlength{\labelwidth}{0.08in}
  \setlength{\labelsep}{0.1in} \setlength{\itemindent}{0in}}}
 {\end{list}}

%\newcommand{\bcar}{\begin{carlist}}
%\newcommand{\ecar}{\end{carlist}}

\newcommand{\bcar}{\begin{itemize}}
\newcommand{\ecar}{\end{itemize}}

\newcommand{\tmpAset}{\ensuremath{\mathbb{L}_0}}
\newcommand{\tmpBset}{\ensuremath{\mathbb{L}_1}} 
\newcommand{\clconv}{\ensuremath{\widebar{\mathrm{conv}}}}


\newcommand{\Constraint}{\ensuremath{\mathcal{C}}}
\newcommand{\hackxi}{z}
\newcommand{\HackXi}{Z}
\newcommand{\hackxitil}{\widetilde{\hackxi}}
\newcommand{\HackXiTil}{\widetilde{\HackXi}}


\newcommand{\matpar}{\ensuremath{\nu}}

\newcommand{\PsiEllOne}{\ensuremath{\Psi_{\ell_1}}}
\newcommand{\PsiHuber}{\ensuremath{\Psi_{\mathrm{Huber}}}}
\newcommand{\HUBERCUT}{\ensuremath{\tau}}


\newcommand{\RealConstraint}{\ensuremath{\mathcal{C}}}

\newcommand{\delstar}{\ensuremath{\delta^*}}

\newcommand{\Fconvex}{\ensuremath{\Fclass_{\mathrm{{conv}}}}}

\newcommand{\SEQTWO}[2]{\ensuremath{(#1_{#2})_{#2=1}^\infty}}
\newcommand{\SEQTHREE}[3]{\ensuremath{(#1_{#2})_{#2=1}^{#3}}}

\newcommand{\Fsparsecone}{\ensuremath{\Fclass_{\mathrm{{spcone}}}}}

%\newcommand{\EYE}[1]{\ensuremath{\mymathbf{I}_{#1 \times #1}}}
\newcommand{\EYE}[1]{\ensuremath{\mymathbf{I}_{#1}}}
\newcommand{\EYETWO}[2]{\ensuremath{\mymathbf{I}_{#1 \times #2}}}
\newcommand{\ZEROMAT}[1]{\ensuremath{\mymathbf{0}_{#1}}}

%\newcommand{\ZeroMat}{\ensuremath{\mymathbf{0}}}

\newcommand{\Fadditive}{\ensuremath{\Fclass_{\mathrm{{add}}}}}
\newcommand{\Fspam}{\ensuremath{\Fclass_{\mathrm{{spam}}}}}

\newcommand{\MCON}{\ensuremath{C}}
\newcommand{\ftrun}{\ensuremath{f_\trunlevel}}



\newcommand{\Ytilspace}{\ensuremath{\widetilde{\Yspace}}}


\newcommand{\delcrittil}{\ensuremath{\widetilde{\delta}_\numobs}}
\newcommand{\delcritstar}{\ensuremath{\delta^*_\numobs}}

\newcommand{\TrunFunT}{\ensuremath{\varphi_\trunlevel}}
\newcommand{\trunlevel}{\ensuremath{\tau}}
\newcommand{\TrunFun}[1]{\ensuremath{\varphi_{#1}}}

\newcommand{\Zn}{\ensuremath{Z_\numobs}}

\newcommand{\HACKCONTWO}{16}

\newcommand{\EQUIVHACKCON}{64}
\newcommand{\Flip}{\ensuremath{\Fclass_{\mathrm{{Lip}}}}}
\newcommand{\Flinear}{\ensuremath{\Fclass_{\mathrm{{lin}}}}}

\newcommand{\Sevent}{\ensuremath{\mathcal{S}}}

\newcommand{\Scal}{\ensuremath{\mathcal{S}}}

\newcommand{\SpecBall}[2]{\ensuremath{\Ball_\numobs(#1; #2)}}



\newcommand{\starhull}[2]{\ensuremath{\mathrm{star}(#1; \, #2)}} 
\newcommand{\plstarhull}[1]{\ensuremath{\mathrm{star}(#1)}}

% Set difference notation
\newcommand{\DIFF}[1]{\ensuremath{\partial #1}}

\newcommand{\Fridge}{\ensuremath{\Fclass_{2}}}
\newcommand{\Fqpar}{\ensuremath{\Fclass_{\qpar}}}

%\newcommand{\SHIFT}[1]{\ensuremath{{#1}_{\fstar}}}
\newcommand{\SHIFT}[1]{\ensuremath{{#1}^*}}

\newcommand{\SEQ}[1]{\ensuremath{(#1)_{j=1}^\infty}}
\newcommand{\RKHS}{reproducing kernel Hilbert space}
\newcommand{\gindex}[1]{\index{general}{#1}}



\newcommand{\indpar}{\ensuremath{\gamma}}


\newcommand{\vhat}{\ensuremath{\widehat{v}}}

\newcommand{\SamCovPert}{\ensuremath{\Pmat}}
\newcommand{\SamCovPertTil}{\ensuremath{\widetilde{\SamCovPert}}}

\newcommand{\pcamult}{\ensuremath{\xi}}



\newcommand{\RWIDTHPL}{\ensuremath{\mathcal{W}}}
\newcommand{\RWIDTH}[1]{\ensuremath{\RWIDTHPL(#1)}}
\newcommand{\RWIDTHSQ}[1]{\ensuremath{\RWIDTHPL^2(#1)}}

\newcommand{\DWIDTHPL}{\ensuremath{D}}
\newcommand{\DWIDTH}[1]{\ensuremath{\DWIDTHPL(#1)}}
\newcommand{\DWIDTHSQ}[1]{\ensuremath{\DWIDTHPL^2(#1)}}

\newcommand{\MYDATA}{\ensuremath{\{x_i\}_{i=1}^\numobs}}
\newcommand{\MVAL}{\ensuremath{\sqrt{M}}}
\newcommand{\MVALSQ}{\ensuremath{M}}

\newcommand{\eigengap}{\ensuremath{\nu}}


% Wedge and vee min and max
%\newcommand{\wmin}{\ensuremath{\wedge}}
%\newcommand{\vmax}{\ensuremath{\vee}}

\newcommand{\GRAPHSAM}[1]{\ensuremath{\{x_i\}_{i=1}^{#1}}}

\newcommand{\TRUNFUN}{\varphi_\trunlev}
\newcommand{\trunlev}{\ensuremath{\tau}}

\newcommand{\ASET}{\ensuremath{\mathbb{A}}}

\newcommand{\missfrac}{\ensuremath{\nu}}

\newcommand{\ThetaINCON}{\ensuremath{\widehat{\ThetaBf}_{\mathrm{{NAI}}}}}

\newcommand{\UNICON}{\ensuremath{c}}

\newcommand{\unicon}{\ensuremath{c}}


%\newcommand{\threshlev}{\ensuremath{\mu_\numobs}}
\newcommand{\threshlev}{\ensuremath{\nu_\numobs}}
\newcommand{\threshtil}{\ensuremath{\widetilde{\mu}_\numobs}}
\newcommand{\opbound}{\ensuremath{\nu_\numobs}}

\newcommand{\ej}{\ensuremath{j}}
\newcommand{\ek}{\ensuremath{k}}
\newcommand{\aind}{\ensuremath{a}}
\newcommand{\bind}{\ensuremath{b}}


\newcommand{\hana}{+}
\newcommand{\ThetaShack}{\ensuremath{\ThetaBf_{\ej \hana}}}
\newcommand{\ThetaShackHat}{\ensuremath{\widehat{\ThetaBf}_{\ej \hana}}}

\newcommand{\thetashack}{\ensuremath{\theta_{\ej \hana}}}
\newcommand{\thetashackhat}{\ensuremath{\widehat{\theta}_{\ej \hana}}}



\newcommand{\clipot}{\ensuremath{\phi}}
\newcommand{\statenum}{\ensuremath{M}}

\newcommand{\Fish}{\ensuremath{\mathbf{J}}}
\newcommand{\FishPlain}{\ensuremath{J}}
\newcommand{\FishStar}{\ensuremath{\Fish^*}}


\newcommand{\GamHat}{\ensuremath{\widehat{\GammaBf}}}
\newcommand{\GamHatPlain}{\ensuremath{\widehat{\Gamma}}}
\newcommand{\PlainGamHat}{\ensuremath{\GamHatPlain}}
\newcommand{\gamhat}{\ensuremath{\widehat{\gamma}}}


\newcommand{\ThetaHackStar}{\ensuremath{\ThetaBf^\diamond}}

\newcommand{\mateltone}[1]{\ensuremath{\|#1\|_{\scriptsize{\ell_1}}}}

\newcommand{\CutSet}{\ensuremath{S}}
\newcommand{\compat}{\ensuremath{\psi}}

\newcommand{\muparn}{\ensuremath{\mu_\numobs}}

\newcommand{\EMPPLAIN}[2]{\ensuremath{\mathcal{E}(#1 \, ; #2)}}
\newcommand{\LossPlain}{\ensuremath{\mathcal{L}}}
\newcommand{\RegOver}[1]{\Regplain_{\mathrm{{over}}}(#1)}


\newcommand{\HACKZSAMP}{\ensuremath{Z}}

% Wedge and vee min and max
\newcommand{\wmin}{\ensuremath{\wedge}}
\newcommand{\vmax}{\ensuremath{\vee}}

\newcommand{\UsubR}{\ensuremath{\Usub^\rdim}}
\newcommand{\VsubR}{\ensuremath{\Vsub^\rdim}}

\newcommand{\fprime}{\ensuremath{\fbar}}
\newcommand{\alphabar}{\ensuremath{\bar{\alpha}}}
\newcommand{\nbar}{\ensuremath{\bar{\numobs}}} 


\newcommand{\omegan}{\ensuremath{\omega_\numobs}}
\newcommand{\omegansq}{\ensuremath{\omega^2_\numobs}}
\newcommand{\omegahat}{\ensuremath{\widehat{\omega}}}

\newcommand{\supp}{\ensuremath{\mathrm{supp}}}

\newcommand{\DelSparse}{\ensuremath{\PertMat_{\Sparse}}}
\newcommand{\DelLowRank}{\ensuremath{\PertMat_{\LowRank}}}
\newcommand{\DelSparseHat}{\ensuremath{\PertMat_{\SparseHat}}}
\newcommand{\DelLowRankHat}{\ensuremath{\PertMat_{\LowRankHat}}}
\newcommand{\atil}{\ensuremath{\tilde{a}}}


\newcommand{\phasecon}{\ensuremath{c_0}}


\newcommand{\prad}{\ensuremath{\sqrt{\pradsq}}}
\newcommand{\pradsq}{\ensuremath{\rho}}


\newcommand{\USEGAM}{\ensuremath{\sqrt{\newgamma}}}
\newcommand{\newgamma}{\widebar{\gamma}}
\newcommand{\newkappa}{\ensuremath{\widebar{\kappa}}}


\newcommand{\TbarSmall}{\ensuremath{\bar{\Tmat}}}
\newcommand{\SUMN}{\ensuremath{\sum_{i=1}^\numobs}}
\newcommand{\SUMNF}{\ensuremath{\frac{1}{\numobs} \SUMN}}



\newcommand{\usedimmin}{\ensuremath{\usedim'}}

\newcommand{\BIGCON}{\ensuremath{C}}



\newcommand{\SEV}{\ensuremath{\sqrt{\frac{ \log \usedim}{\numobs}}}}
\newcommand{\SevVar}{\ensuremath{T}}
\newcommand{\lrad}{\ensuremath{r_\ell}}
\newcommand{\urad}{\ensuremath{r_u}}
\newcommand{\ESEV}{\ensuremath{2}}

\newcommand{\myemphparagraph}[1]{\noindent \emph{#1}}
\newcommand{\mybfparagraph}[1]{\noindent {\bf{#1}}}

\newcommand{\SpecSset}{\ensuremath{\mathbb{S}}}
\newcommand{\SHORTQ}{\ensuremath{\Qmat}}
\newcommand{\SpecSetTil}{\ensuremath{\widetilde{\SpecSet}}}
\newcommand{\SpecSsetTil}{\ensuremath{\widetilde{\SpecSset}}}



\newcommand{\myeigval}{\ensuremath{\gamma}}
\newcommand{\mysingval}{\ensuremath{\sigma}}

\newcommand{\mylammax}{\ensuremath{\myeigval_{\mathrm{{max}}}}}
\newcommand{\mylammin}{\ensuremath{\myeigval_{\mathrm{{min}}}}}
\newcommand{\myxsam}{\ensuremath{x}}
\newcommand{\CEXP}[1]{\ensuremath{e^{#1}}}
\newcommand{\LOWCEXP}[1]{\ensuremath{ \exp \left ( {#1} \right) }}
\newcommand{\CEXPBIG}[1]{\ensuremath{\exp \left(#1 \right)}}
\newcommand{\CEXPSUPERBIG}[1]{\ensuremath{\exp \left(#1 \right)}}
\newcommand{\matlam}{\ensuremath{\lambda}}
\newcommand{\mytrace}[1]{\ensuremath{\operatorname{tr} (#1)}}

% Matrix regression X
\newcommand{\mrX}{\ensuremath{\Zmat}}



%\newcommand{\atil}{\ensuremath{a}}

\newcommand{\maxval}{\ensuremath{\alpha}}
\newcommand{\rscprecon}{\ensuremath{c_0}}
\newcommand{\HACK}{\ensuremath{\mathcal{K}}}
\newcommand{\DALCON}{\ensuremath{\ALCON}}
\newcommand{\ALCON}{\ensuremath{\alpha}}
\newcommand{\FERRSQ}[2]{\ensuremath{e^2(#1, \, #2)}}
\newcommand{\EventTil}{\ensuremath{\widetilde{\Event}}}


% Special notation for multivariate regression, number of predictors
\newcommand{\mrusedim}{\ensuremath{p}}

\newcommand{\MatA}{\ensuremath{\alpha}}
\newcommand{\MatB}{\ensuremath{\beta}}
\newcommand{\DeltaA}{\ensuremath{\Delta_\MatA}}
\newcommand{\DeltaB}{\ensuremath{\Delta_\MatB}}

\newcommand{\MatATil}{\ensuremath{\widebar{\MatA}}}
\newcommand{\MatBTil}{\ensuremath{\widebar{\MatB}}}

\newcommand{\SUPERSUB}{\ensuremath{\ModelSetOver(\BigSgroup)}}

\newcommand{\Row}{\ensuremath{\mathbf{\RowPlain}}}
\newcommand{\RowHat}{\ensuremath{\widehat{\Row}}}
\newcommand{\RowPlain}{\ensuremath{\Omega}}

\newcommand{\SUBA}{\ensuremath{\mathbb{M}_\MatA}}
\newcommand{\SUBB}{\ensuremath{\mathbb{M}_\MatB}}
\newcommand{\SUBAPERP}{\ensuremath{\SUBA^\perp}}
\newcommand{\SUBBPERP}{\ensuremath{\SUBB^\perp}}

\newcommand{\MatDecompNorm}[1]{\ensuremath{\Phi_{\omega}(#1)}}

\newcommand{\MatDecompNormSq}[1]{\ensuremath{\Phi^2_{\omega}(#1)}}

\newcommand{\smallxbar}{\ensuremath{\bar{x}}}

\newcommand{\sval}{\ensuremath{\mysingval}}


\newcommand{\Nrad}{\ensuremath{r}} 
\newcommand{\nradone}{\ensuremath{\Nrad_1}}
\newcommand{\nradtwo}{\ensuremath{\Nrad_2}}

\newcommand{\Lvar}{\ensuremath{Q}}


\newcommand{\sym}{\ensuremath{\operatorname{sym}}}

\newcommand{\rnum}{\ensuremath{r}}

%\newcommand{\BigSgroup}{\ensuremath{\Sset_{\mathrm{{group}}}}}
%\newcommand{\BigSgroupTil}{\ensuremath{\widetilde{\Sset}_{\mathrm{{group}}}}}


\newcommand{\BigSelt}{\ensuremath{\Sset_{\mathrm{{elt}}}}}

\newcommand{\BigSgroup}{\ensuremath{\Sset_\Group}}
\newcommand{\BigSgroupTil}{\ensuremath{\widetilde{\Sset}_{\Group}}}



\newcommand{\Good}{\ensuremath{\mathbb{G}}}

\newcommand{\PiMat}{\ensuremath{\mathbf{\Pi}}}

\newcommand{\PINC}[1]{\ensuremath{\delta_{\mathrm{{PW}}}(#1)}}
\newcommand{\perthat}{\ensuremath{\widehat{\perturb}}}


\newcommand{\lweight}{\ensuremath{\nu}}
\newcommand{\wellone}[1]{\ensuremath{\|#1\|_{\lweight(1)}}}
\newcommand{\wellinfty}[1]{\ensuremath{\|#1\|_{\lweight(\infty)}}}

\newcommand{\NewCset}{\ensuremath{\mathbb{T}}}

\newcommand{\ZmatHat}{\ensuremath{\widehat{\Zmat}}}

\newcommand{\Tbset}{\ensuremath{\mathbb{T}}}

\newcommand{\tworad}{\ensuremath{R}}
\newcommand{\twourad}{\ensuremath{\tworad_u}}
\newcommand{\twolrad}{\ensuremath{\tworad_\ell}}
\newcommand{\ANNOYPEEL}{\ensuremath{M_\numobs(\RegPlain; \tworad)}}


\newcommand{\Aset}{\ensuremath{\mathbb{A}}}

\newcommand{\RIP}[1]{\ensuremath{\delta_{#1}}}

\newcommand{\PlainReg}{\RegPlain}
\newcommand{\TayErrSing}{\ensuremath{\mathcal{E}}}
\newcommand{\TaySing}{\ensuremath{\TayErrSing}}

\newcommand{\EMPTAYPLAIN}{\ensuremath{\delLike}}
\newcommand{\POPTAYPLAIN}{\ensuremath{\delLikeBar}}
\newcommand{\EMPTAY}[1]{\ensuremath{\delLike(#1)}}
\newcommand{\POPTAY}[1]{\ensuremath{\delLikeBar(#1)}}

\newcommand{\SYM}[1]{\ensuremath{\mbox{sym}(#1)}}

\newcommand{\MYSCORE}[1]{\ensuremath{\nabla \Loss(#1)}}
\newcommand{\MYLOSS}[1]{\ensuremath{\Loss(#1)}}
\newcommand{\MYLOSSBAR}[1]{\ensuremath{\LossBar(#1)}}

\newcommand{\tbar}{\ensuremath{\widebar{t}}}

\newcommand{\LinkBound}{\ensuremath{B}}

\newcommand{\MYDUALREG}{\ensuremath{\mu_\numobs(\RegPlain^*)}}
\newcommand{\MYDUALREGSQ}{\ensuremath{\mu^2_\numobs(\RegPlain^*)}}

\newcommand{\PlainCovMat}{\ensuremath{\Sigma}}

\newcommand{\bspikeplain}{\ensuremath{\alpha}}
\newcommand{\nrad}{\ensuremath{\rho}}

\newcommand{\MYMAX}[2]{\ensuremath{\max\{#1, \, #2\}}}
\newcommand{\MYMAXX}[2]{\ensuremath{\max \left\{#1, \, #2 \right\}}}
\newcommand{\MYMIN}[2]{\ensuremath{\min\{#1, \, #2\}}}
\newcommand{\MYMINN}[2]{\ensuremath{\min \left\{#1, \, #2 \right\}}}
%\newcommand{\MYMIN}[2]{\ensuremath{ \{ #1 \wedge #2 \}}}

\newcommand{\BUHL}{\index{author}{B\"{u}hlmann, P.}}
\newcommand{\GEER}{\index{author}{van de Geer, S.}}
\newcommand{\CANDES}{\index{author}{Candes, E.}}
\newcommand{\TAO}{\index{author}{Tao, T.}}
\newcommand{\DON}{\index{author}{Donoho, D.}}

\newcommand{\ObsZ}{\ensuremath{Z}}
\newcommand{\BadEvent}{\ensuremath{\mathcal{E}}}
\newcommand{\BadEventZero}{\ensuremath{\BadEvent_0}}
\newcommand{\BadEventOne}{\ensuremath{\BadEvent_1}}



\newcommand{\Poly}{\ensuremath{\mathcal{P}}}





\newcommand{\subexpvarstar}{\ensuremath{\nu_*}}


\newcommand{\xprime}{\ensuremath{x'}}
\newcommand{\FrancisSet}{\ensuremath{\mathbb{S}}}

\newcommand{\usedimmax}{\ensuremath{\usedim{\,'}}}

\newcommand{\betaspike}{\ensuremath{\alpha_{\mathrm{{sp}}}}}

\newcommand{\CovMatHat}{\ensuremath{\widehat{\CovMat}}}

\newcommand{\thetamin}{\ensuremath{\theta_{\mathrm{{min}}}}}
\newcommand{\thetaminsq}{\ensuremath{\theta^2_{\mathrm{{min}}}}}
\newcommand{\thetabar}{\widebar{\theta}}

\newcommand{\mprobbar}{\ensuremath{\bar{\mprob}}}
\newcommand{\qprobbar}{\ensuremath{\bar{\qprob}}}

\newcommand{\SPEC}{\ensuremath{K}}
\newcommand{\SPECSQ}{\ensuremath{\SPEC^2}}

\newcommand{\qprobbarn}{\ensuremath{\widebar{\qprob}^\numobs}}

\newcommand{\Hrandvar}{\ensuremath{Z}}
\newcommand{\HrandSpace}{\ensuremath{\mathcal{Z}}}
\newcommand{\hvalue}{\ensuremath{z}}

\newcommand{\qprobone}{\ensuremath{\qprob_1}}
\newcommand{\qprobtwo}{\ensuremath{\qprob_2}}

\newcommand{\Jrand}{\ensuremath{\Jrandpl_\delta}}
\newcommand{\Jrandpl}{\ensuremath{J}}

\newcommand{\MinFun}{\ensuremath{\Phi}}
\newcommand{\MYEXP}[1]{\ensuremath{\exp \left({#1} \right)}}
\newcommand{\MYEXPUP}[1]{\ensuremath{e^{#1}}}

\newcommand{\Emask}{\ensuremath{E}}

\newcommand{\GenSub}{\ensuremath{\mathbb{S}}}

\newcommand{\GamBar}{\ensuremath{\bar{\Gamma}}}

\newcommand{\vect}{\ensuremath{\mbox{vec}}}

\newcommand{\MYMCON}{\ensuremath{\frac{\NewMcon}{2}}}

\newcommand{\NewMconPrime}{\ensuremath{\widebar{\NewMcon}}}
\newcommand{\NewMconPrimeSmall}{\ensuremath{\bar{\NewMcon}}}

\newcommand{\ThetaBad}{\ensuremath{\ThetaBf^{\mathrm{{bad}}}}}

\newcommand{\PertGood}{\ensuremath{\PertMat_{\mathrm{{good}}}}}
\newcommand{\PertBad}{\ensuremath{\PertMat_{\mathrm{{bad}}}}}
\newcommand{\pertgood}{\ensuremath{\perturb_{\mathrm{{good}}}}}
\newcommand{\pertbad}{\ensuremath{\perturb_{\mathrm{{bad}}}}}
\newcommand{\TELE}{\ensuremath{\PLAINTELE(\CovMat)}}
\newcommand{\TELESQRT}{\ensuremath{\PLAINTELESQRT(\CovMat)}}
\newcommand{\PLAINTELE}{\ensuremath{\rho^2}}
\newcommand{\PLAINTELESQRT}{\ensuremath{\rho}}

\newcommand{\SPLINONE}{(G1)} 
\newcommand{\SPLINONEPRIME}{(G1$'$)} 
\newcommand{\SPLINTWO}{(G2)} 


\newcommand{\stepsize}{\ensuremath{\alpha}}
\newcommand{\RegPlain}{\ensuremath{\Phi}}

\newcommand{\Vset}{\ensuremath{\mathcal{V}}}

%\newcommand{\Usub}{\ensuremath{\mathcal{U}}}
%\newcommand{\Vsub}{\ensuremath{\mathcal{V}}}
\newcommand{\Usub}{\ensuremath{\mathbb{U}}}
\newcommand{\Vsub}{\ensuremath{\mathbb{V}}}


\newcommand{\colsp}{\ensuremath{\colspan}}
\newcommand{\rowsp}{\ensuremath{\rowspan}}


\newcommand{\colspan}{\ensuremath{\mbox{colspan}}}
\newcommand{\rowspan}{\ensuremath{\mbox{rowspan}}}

\newcommand{\tasknum}{\ensuremath{T}}
\newcommand{\numtask}{\ensuremath{T}}

\newcommand{\bigN}{\ensuremath{N}}

\newcommand{\zhangslop}{\ensuremath{\tau_\numobs}}
\newcommand{\zhangcurve}{\ensuremath{\NewMcon}}
\newcommand{\zhangrad}{\ensuremath{R}}


\newcommand{\subgauss}{\ensuremath{\sigma}}

\newcommand{\SUPERCONEPLAIN}{\ensuremath{\ConeSet(\ModelSet,
\ModelSetPerp)}}

\newcommand{\SUPERCONE}{\ensuremath{\ConeSet_{\tparam}(\ModelSet,
\BsetPerp)}}

% Expected value of dual norm (in ChapterDecomposable)
\newcommand{\CUPPA}{\ensuremath{c_\numobs(\Regdplain)}}

% Annoying hacking commands
\newcommand{\SERENA}{\ensuremath{\theta^*_{\ModelSetPerp}}}
\newcommand{\SERENAMODEL}{\ensuremath{\theta^*_{\ModelSet}}}

% Generic subspace
\newcommand{\SubSpace}{\ensuremath{{\mathbb{S}}}}
\newcommand{\NewSubSpace}{\ensuremath{{\mathbb{V}}}}

% Length of a time series
\newcommand{\Tlength}{\ensuremath{N}}

\newcommand{\Avar}{\ensuremath{A}}
\newcommand{\Zvar}{\ensuremath{Z}}
\newcommand{\zvar}{\ensuremath{z}}

\newcommand{\xbar}{\ensuremath{\widebar{x}}}

\newcommand{\GenErr}[1]{\ensuremath{\| #1\|}}
\newcommand{\GenErrSq}[1]{\ensuremath{\| #1\|^2}}



\newcommand{\Cset}{\ensuremath{\mathbb{C}}}

%\newcommand{\gmax}{\ensuremath{g_{\mathrm{{max}}}}}
\newcommand{\gmax}{\ensuremath{m}}

\newcommand{\group}{\ensuremath{g}}
\newcommand{\hgroup}{\ensuremath{h}}
\newcommand{\Group}{\ensuremath{\mathcal{G}}}
\newcommand{\groupnum}{\ensuremath{T}}
\newcommand{\Sgroup}{\ensuremath{\mathcal{S}}}
\newcommand{\SgroupBar}{\ensuremath{\Sgroup^c}}
\newcommand{\BigSgroupBar}{\ensuremath{\BigSgroup^c}}
\newcommand{\SgroupTil}{\ensuremath{\widetilde{\Sgroup}}}


\newcommand{\pval}{\ensuremath{p}}
\newcommand{\qval}{\ensuremath{q}}

\newcommand{\LinkFun}{\ensuremath{\psi}}
\newcommand{\LinkFunTwo}{\ensuremath{\LinkFun''}}

\newcommand{\betahatlam}{\ensuremath{\widehat{\betapar}_{\regpar}}}





\newcommand{\HACKER}{\ensuremath{9 \, \LipCon}}
\newcommand{\trad}{\ensuremath{r}}
\newcommand{\AVAR}{\ensuremath{A}}
\newcommand{\BVAR}{\ensuremath{B}}
\newcommand{\CVAR}{\ensuremath{C}}



\newcommand{\BigProjModel}[1]{\ensuremath{\Pi_{\ModelSet}(#1)}}
\newcommand{\BigProjModelPerp}[1]{\ensuremath{\Pi_{\ModelSet^\perp}(#1)}}
\newcommand{\BigProjBset}[1]{\ensuremath{\Pi_{\BsetSmall}(#1)}}
\newcommand{\BigProjBsetPerp}[1]{\ensuremath{\Pi_{\BsetSmallPerp}(#1)}}

\newcommand{\ProjModel}[1]{#1_{\ModelSet}}
\newcommand{\ProjModelPerp}[1]{#1_{\ModelSet^\perp}}
\newcommand{\ProjBset}[1]{#1_{\BsetSmall}}
\newcommand{\ProjBsetPerp}[1]{#1_{\BsetSmall^\perp}}

\newcommand{\betapar}{\ensuremath{\theta}}


\newcommand{\BigReg}[1]{\ensuremath{\Regplain \left(#1 \right)}}

\newcommand{\RSC}{\ensuremath{\operatorname{RSC}}}

\newcommand{\pdima}{\ensuremath{{\pdim_1}}}
\newcommand{\pdimb}{\ensuremath{{\pdim_2}}}
\newcommand{\Apperr}{\ensuremath{\mathcal{E}_{\operatorname{app}}}}
\newcommand{\Esterr}{\ensuremath{\mathcal{E}_{\operatorname{err}}}}
\newcommand{\Nullerr}{\ensuremath{\mathcal{E}_{\operatorname{null}}}}
\newcommand{\SuperConvSet}{\ensuremath{\ConvSet(\ModelSet, \Bset;
    \thetastar)}}
\newcommand{\SuperKeySet}{\ensuremath{\KeySet(\ErrRad; \ModelSet,
    \Bset, \thetastar)}}

\newcommand{\SuperRSC}{\ensuremath{ \RSC(\epsilon, \NewMcon;
    \ModelSet, \BsetPerp)}}

\newcommand{\Stau}{\ensuremath{\Sset_\taupar}}

\newcommand{\Gfun}{\ensuremath{\mathcal{F}}}

\newcommand{\TmpVarA}{\ensuremath{\alpha}}
\newcommand{\TmpVarB}{\ensuremath{\beta}}

%\newcommand{\Regplain}{\ensuremath{\mathcal{R}}}

\newcommand{\Regplain}{\ensuremath{\Phi}}

\newcommand{\Regd}[1]{\ensuremath{\Regplain^*(#1)}}
\newcommand{\Regdplain}{\ensuremath{\Regplain^*}}

\newcommand{\Reg}[1]{\ensuremath{\Regplain(#1)}}
\newcommand{\RegSq}[1]{\ensuremath{\Regplain^2(#1)}}


\newcommand{\ModelSet}{\ensuremath{\mathbb{M}}}
\newcommand{\ModelSetPerp}{\ensuremath{\ModelSet^\perp}}

\newcommand{\Bset}{\widebar{\ModelSet}}
\newcommand{\BsetSmall}{\bar{\ModelSet}}
\newcommand{\BsetPerp}{\Bset^\perp}
\newcommand{\BsetSmallPerp}{\BsetSmall^\perp}



\newcommand{\ConvSet}{\ensuremath{\mathbb{C}}}
\newcommand{\KeySet}{\mathbb{K}}



\newcommand{\delpar}{\ensuremath{\Delta}}
\newcommand{\delparhat}{\ensuremath{\widehat{\delpar}}}



\newcommand{\TINYO}{{\ensuremath{\mathrm{{O}}}}}
\newcommand{\TINYOO}{{\ensuremath{\mathrm{{OO}}}}}
\newcommand{\TINYH}{{\ensuremath{\mathrm{{H}}}}}
\newcommand{\TINYHH}{{\ensuremath{\mathrm{{HH}}}}}



%\newcommand{\LowRank}{\ensuremath{L}}

\newcommand{\LowRankHat}{\ensuremath{\widehat{\LowRank}}}
\newcommand{\SparseHat}{\ensuremath{\widehat{\Sparse}}}
\newcommand{\regparone}{\ensuremath{\regparn}}
\newcommand{\regpartwo}{\ensuremath{\mu_\numobs}}


\newcommand{\rdim}{\ensuremath{r}}

\newcommand{\astar}{\ensuremath{a^*}}

\newcommand{\Wstil}{\ensuremath{\tilde{\Wmat}}}

\newcommand{\CovBound}{\ensuremath{b}}
\newcommand{\RON}{\ensuremath{7}}

\newcommand{\ahat}{\ensuremath{\widehat{a}}}


\newcommand{\sminus}{\ensuremath{s^{\scriptsize{-}}}}
\newcommand{\sback}{\ensuremath{\backslash \{\ej\}}}

\newcommand{\ntheta}[1]{\ensuremath{\theta^{#1}}}
\newcommand{\xnot}[1]{\ensuremath{x_{\backslash \{#1\}}}}
\newcommand{\Xnot}[1]{\ensuremath{\Xmat_{\backslash \{#1\}}}}
\newcommand{\XnotPlain}[1]{\ensuremath{X_{\backslash \{#1\}}}}
\newcommand{\XnotData}[2]{\ensuremath{\Xmat_{#1 \backslash \{#2\}}}}
\newcommand{\xnotdata}[2]{\ensuremath{x_{#1 \backslash \{#2\}}}}
\newcommand{\Znot}[1]{\ensuremath{Z_{\backslash \{#1\}}}}
\newcommand{\ZnotSmall}[1]{\ensuremath{z_{\backslash \{#1\}}}}

\newcommand{\Wme}[1]{\ensuremath{W_{#1}}}


\newcommand{\nthetas}[2]{\ensuremath{\theta^{#1}_{#2}}}
\newcommand{\Xnots}[2]{\ensuremath{X_{#2; \backslash \{#1\}}}}
\newcommand{\Wnots}[2]{\ensuremath{W_{#2; \backslash \{#1\}}}}

\newcommand{\vinda}{\ensuremath{s}}


%\newcommand{\degmax}{\ensuremath{\rho}}
%\newcommand{\degmax}{\ensuremath{D}}
%\newcommand{\degmax}{\ensuremath{k}}
\newcommand{\degmax}{\ensuremath{m}}

\newcommand{\PHIQ}{\ensuremath{\varphi(\qprob, \sigma_w)}}

\newcommand{\GamStar}{\ensuremath{\GammaBf^*}}

%\newcommand{\OffNorm}[1]{\ensuremath{\| #1 \|_{\mathrm{{1,off}}}}}
%\newcommand{\OffNormMax}[1]{\ensuremath{\| #1 \|_{\mathrm{{max,off}}}}}

\newcommand{\OffNormMax}[1]{\ensuremath{\matsnorm{#1}{\mathrm{{max,off}}}}}
\newcommand{\OffNorm}[1]{\ensuremath{\matsnorm{#1}{\mathrm{{1,off}}}}}


\newcommand{\neigh}{\ensuremath{\mathcal{N}}}
\newcommand{\neighplus}{\ensuremath{\neigh^+}}
\newcommand{\neighhat}{\ensuremath{\widehat{\neigh}}}

% Notation for an image vector (compressed sensing)
\newcommand{\image}{\ensuremath{\beta}}


\newcommand{\LogLike}{\ensuremath{\ell}}

%\newcommand{\Data}{\ensuremath{X_1^\numobs}}

\newcommand{\expcompat}{\ensuremath{\psi}}

\newcommand{\ENCMIN}[1]{\ensuremath{\left\{ #1 \right\}}}

\newcommand{\Xop}{\ensuremath{\mathfrak{X}_\numobs}}

\newcommand{\Sparse}{\ensuremath{\GammaBf}}
\newcommand{\PlainSparse}{\ensuremath{\Gamma}}
\newcommand{\SparsePlain}{\ensuremath{\Gamma}}
\newcommand{\LowRank}{\ensuremath{\LambdaBf}}
\newcommand{\PlainLowRank}{\ensuremath{\Lambda}}
\newcommand{\TrueSparse}{\ensuremath{\Sparse^*}}
\newcommand{\TrueLowRank}{\ensuremath{\LowRank^*}}

\newcommand{\PlainTrueSparse}{\ensuremath{\PlainSparse^*}}
\newcommand{\PlainTrueLowRank}{\ensuremath{\PlainLowRank^*}}
\newcommand{\PlainSparseHat}{\ensuremath{\widehat{\PlainSparse}}}
\newcommand{\PlainLowRankHat}{\ensuremath{\widehat{\PlainLowRank}}}


\newcommand{\CliqueSet}{\ensuremath{\mathfrak{C}}}

\newcommand{\condind}{\ensuremath{\perp\!\!\!\perp}}

\newcommand{\Plaincon}{\ensuremath{C}}

\newcommand{\blinvec}{\ensuremath{\beta}}
\newcommand{\Fsparse}{\Fclass_{\mathrm{{spar}}}}

\newcommand{\PolyClass}{\ensuremath{\mathcal{P}}}

\newcommand{\phitil}{\ensuremath{\widetilde{\phi}}}

\newcommand{\Fortho}{\ensuremath{\Fclass_{\mathrm{{ortho}}}}}
\newcommand{\FclassT}[1]{\ensuremath{\Fortho(#1; T)}}

\newcommand{\IID}{i.i.d.~}
\newcommand{\IIDNOSPACE}{i.i.d.}
\newcommand{\ER}{Erd\"{o}s--R\'{e}nyi}

\newcommand{\Fconv}{\ensuremath{\Fclass_{\mathrm{{conv}}}}}
\newcommand{\boutil}{\ensuremath{\tilde{\bou}}}

%\newcommand{\LOW}{\ensuremath{\eta}}
\newcommand{\LOW}{\ensuremath{\nu}}

\newcommand{\ChelHat}{\ensuremath{\widehat{Z}_\numobs}}
\newcommand{\Chel}{\ensuremath{\widebar{Z}_\numobs}}


\newcommand{\SAM}[2]{\ensuremath{\mathcal{C}({#1},{#2})}}
\newcommand{\LipCon}{\ensuremath{L}}




%\newcommand{\MYLOSS}[1]{\ensuremath{\Loss_{#1}}}
\newcommand{\HACKLOSS}[1]{\ensuremath{\LossSing_{#1}}}
\newcommand{\QUADFUN}{\ensuremath{\mathcal{Q}}}

%\newcommand{\Curv}{\ensuremath{C}}
\newcommand{\Curv}{\ensuremath{\gamma}}

\newcommand{\DELTA}[1]{\ensuremath{\HACKLOSS{#1} - \HACKLOSS{\fstar}}} 


\newcommand{\TINYLIP}{\ensuremath{\mathrm{{Lip}}}} 
\newcommand{\TINYAND}{\ensuremath{\mathrm{{AND}}}} 
\newcommand{\TINYOR}{\ensuremath{\mathrm{{OR}}}} 


\newcommand{\LocRadPop}{\ensuremath{\widebar{\mathcal{R}}_\numobs}}
\newcommand{\LocRadPopSmall}{\ensuremath{\bar{\mathcal{R}}_\numobs}}

\newcommand{\Aevent}{\ensuremath{\mathcal{A}}}

\newcommand{\Bevent}{\ensuremath{\mathcal{B}}}

\newcommand{\FUNNORM}[2]{\ensuremath{\matsnorm{#1}{#2}}}

\newcommand{\Xhack}[1]{\ensuremath{X^{#1}}}
\newcommand{\xhack}[1]{\ensuremath{x^{#1}}}

\newcommand{\Yhack}[1]{\ensuremath{Y^{#1}}}
\newcommand{\yhack}[1]{\ensuremath{y^{#1}}}

\newcommand{\Zhack}[1]{\ensuremath{Z^{#1}}}
\newcommand{\zhack}[1]{\ensuremath{z^{#1}}}

\newcommand{\SpecConeSub}[2]{\ensuremath{\ConeSub_{#2}(#1)}}

\newcommand{\Can}[1]{\ensuremath{\Delta^{#1}}}

\newcommand{\cprob}{\ensuremath{\mathbb{M}}}
\newcommand{\cdens}{\ensuremath{m}}

\newcommand{\LAUR}{\ensuremath{c}}

\newcommand{\LaurentBset}{\ensuremath{\mathcal{B}}}



\newcommand{\xannoy}[1]{\ensuremath{x_{#1}}}
\newcommand{\yannoy}[1]{\ensuremath{y_{#1}}}
\newcommand{\Xannoy}[1]{\ensuremath{X_{#1}}}
\newcommand{\Yannoy}[1]{\ensuremath{Y_{#1}}}

%\newcommand{\Shannon}{\ensuremath{\mathbb{S}}}
\newcommand{\Shannon}{\ensuremath{H}}

\newcommand{\PSIFUN}{\ensuremath{\psi}}


\newcommand{\realplus}{\ensuremath{\real_+}}


\newcommand{\GoodEnt}{\ensuremath{\mathbb{H}}}
\newcommand{\ELAMX}{\ensuremath{e^{\lambda X}}}
\newcommand{\MOM}{\ensuremath{\varphi}}
\newcommand{\CUM}{\ensuremath{\Phi}}
\newcommand{\MOMX}{\ensuremath{\varphi_{\mathrm{x}}}}
\newcommand{\MOMXTIL}{\ensuremath{\varphi_{\mathrm{\tilde{x}}}}}



\newcommand{\PhiMap}{\ensuremath{\Phi}}
\newcommand{\kereig}{\ensuremath{\mu}}
\newcommand{\kereighat}{\ensuremath{\widehat{\kereig}}}

\newcommand{\LINSP}{\ensuremath{\widetilde{{\mathbb{H}}}}}
\newcommand{\plainin}[2]{\ensuremath{\inprod{#1}{#2}_{\LINSP}}}


\newcommand{\Null}{\ensuremath{\mathbb{N}}}

\newcommand{\Lin}{\ensuremath{L}}
\newcommand{\smoothpar}{\ensuremath{\alpha}}

\newcommand{\xtil}{\ensuremath{\widetilde{x}}}

\newcommand{\pdeg}{\ensuremath{\polydeg}}

\newcommand{\HilRad}{\ensuremath{R}}

\newcommand{\linvec}{\ensuremath{\theta}}
\newcommand{\linvecstar}{\ensuremath{\linvec^*}}
\newcommand{\linvechat}{\ensuremath{\widehat{\linvec}}}



\newcommand{\LinSpace}{\ensuremath{\mathbb{L}}}


\newcommand{\MyCost}{\ensuremath{\mathcal{C}}}



\newcommand{\PsiMat}{\ensuremath{\mathbf{\Psi}}}

\newcommand{\PertMat}{\ensuremath{\mathbf{\Delta}}}
\newcommand{\pertmat}{\ensuremath{p}}
\newcommand{\PertMatTil}{\ensuremath{\widetilde{\PertMat}}}
\newcommand{\pertmattil}{\ensuremath{\tilde{\pertmat}}}
\newcommand{\thetahatsm}{\ensuremath{\hat{\theta}}}
\newcommand{\mywbar}{\ensuremath{\bar{w}}}
\newcommand{\HACKC}{\ensuremath{r}}
%\newcommand{\MatUp}{\ensuremath{\widehat{\Gamma}}}
\newcommand{\MatUp}{\ensuremath{\SamCovPert_3}}
\newcommand{\tailpar}{\ensuremath{\delta}}
\newcommand{\etain}{\ensuremath{\varrho}}
\newcommand{\orthvec}{\ensuremath{\xi}}
\newcommand{\PLAINCON}{\ensuremath{C}}
\newcommand{\HACKREG}{\ensuremath{\Phi_{\scriptsize{\regparn}}}}
\newcommand{\SamTil}{\ensuremath{\widetilde{\Sigma}}}
\newcommand{\ShanghaiPsi}{\ensuremath{\Psi}}
\newcommand{\clam}{\ensuremath{\plaincon_\regpar}}
\newcommand{\regparnsq}{\ensuremath{\regpar^2_\numobs}}
\newcommand{\NOISEFUN}{\ensuremath{\varphi_\eigengap}}
\newcommand{\NOISEFUNTWO}{\ensuremath{\psi_\eigengap}}

\newcommand{\rscslop}{\tau^2_\numobs}
\newcommand{\rscslopsq}{\tau^2_\numobs}

\def\loss{\Loss} 
\def\gradloss{\nabla \loss} 
\def\tparam{\theta^{*}}



\newcommand{\ConeSet}{\ensuremath{\mathbb{C}}}
\newcommand{\twoafun}{\ensuremath{\ddot{A}}}





\newcommand{\Vtil}{\ensuremath{\widetilde{V}}}

\newcommand{\Dhat}{\ensuremath{\widehat{D}}}
\newcommand{\DmatHat}{\ensuremath{\widehat{\Dmat}}}

\newcommand{\BauxEvent}{\ensuremath{\mathcal{B}}}

\newcommand{\GammaBf}{\ensuremath{\mathbf{\Gamma}}}
\newcommand{\PhiBf}{\ensuremath{\mathbf{\Phi}}}
\newcommand{\LambdaBf}{\ensuremath{\mathbf{\Lambda}}}
\newcommand{\SigmaBf}{\ensuremath{\mathbf{\Sigma}}}

\newcommand{\ThetaStar}{\ensuremath{\ThetaBf^*}}
\newcommand{\ThetaStarPlain}{\ensuremath{\Theta^*}}
\newcommand{\ThetaHat}{\ensuremath{\widehat{\ThetaBf}}}
\newcommand{\ThetaHatPlain}{\ensuremath{\widehat{\Theta}}}
\newcommand{\ThetaTil}{\ensuremath{\widetilde{\ThetaBf}}}
\newcommand{\PlainThetaTil}{\ensuremath{\widetilde{\Theta}}}
\newcommand{\PlainThetaHat}{\ensuremath{\widehat{\Theta}}}

\newcommand{\SigHat}{\ensuremath{\widehat{\CovMat}}}


\newcommand{\Fnorm}[1]{\ensuremath{\|#1\|_{\Fclass}}}
\newcommand{\regparn}{\ensuremath{{\regpar_{\numobs}}}}
\newcommand{\regparnhalf}{\ensuremath{\frac{\regparn}{2}}}

\newcommand{\JointCost}{\ensuremath{\phi}}
\newcommand{\DelTil}{\ensuremath{\widetilde{\Delta}}}
\newcommand{\DelStar}{\ensuremath{\Delta^*}}

\newcommand{\delhat}{\estim{\delpar}}


% General noise for non-parametric regression
\newcommand{\gennoise}[1]{\ensuremath{\varepsilon_{#1}}}

\newcommand{\DelHat}{\ensuremath{\widehat{\Delta}}}
\newcommand{\hilnorm}[1]{\ensuremath{\|#1\|_{\Hil}}}
\newcommand{\hilin}[2]{\ensuremath{\inprod{#1}{#2}_{\Hil}}}


\newcommand{\HilSub}{\ensuremath{\mathbb{J}}}
\newcommand{\ghat}{\ensuremath{\widehat{g}}}

% Rescaled kernel function
\newcommand{\Kernew}{\ensuremath{K}}
\newcommand{\CritFun}{\ensuremath{F}}




\newcommand{\Pclass}{\ensuremath{\mathcal{P}}}
\newcommand{\Pzero}{\ensuremath{\Pclass_0}}
\newcommand{\Pone}{\ensuremath{\Pclass_1}}
\newcommand{\mprobone}{\ensuremath{\mprob_1}}
\newcommand{\mprobzero}{\ensuremath{\mprob_0}}

\newcommand{\mprobn}{\ensuremath{\mprob^{1:\numobs}}}
\newcommand{\qprobn}{\ensuremath{\qprob^{1:\numobs}}}
\newcommand{\uprobn}{\ensuremath{\uprob^{1:\numobs}}}



\newcommand{\Fdiv}[2]{\ensuremath{D_f(#1 \, \| \, #2)}}
\newcommand{\Vdist}[2]{\ensuremath{V(#1 \, \| \, #2)}}
\newcommand{\Hell}[2]{\ensuremath{H(#1 \, \| \, #2)}}
\newcommand{\HellSq}[2]{\ensuremath{H^2(#1 \, \| \, #2)}}
\newcommand{\BigHellSq}[2]{\ensuremath{H^2 \left(#1 \, \| \, #2 \right)}}
\newcommand{\ChiSq}[2]{\ensuremath{\chi^2(#1 \, \| \, #2)}}


\newcommand{\Mpack}{\ensuremath{M}}
\newcommand{\MpackPlain}{\ensuremath{M}}
\newcommand{\MpackDelta}{\ensuremath{\Mpack(2 \delta)}}

\newcommand{\perr}{\ensuremath{q_e}}
\newcommand{\psistar}{\ensuremath{\psi^*}}

\newcommand{\Aclass}{\ensuremath{\mathcal{A}}}
\newcommand{\Bclass}{\ensuremath{\mathcal{B}}}
\newcommand{\uprob}{\ensuremath{\mathbb{U}}}



\newcommand{\smooth}{\ensuremath{M}}

\newcommand{\sparsedim}{\ensuremath{s}}

\newcommand{\gamlow}{\ensuremath{\eta_{\ell}}}
\newcommand{\gamup}{\ensuremath{\eta_{u}}}
\newcommand{\gammin}{\ensuremath{\eta_{\mathrm{{min}}}}}
\newcommand{\gammax}{\ensuremath{\eta_{\mathrm{{max}}}}}

\newcommand{\gamminsq}{\ensuremath{\eta^2_{\mathrm{{min}}}}}
\newcommand{\gammaxsq}{\ensuremath{\eta^2_{\mathrm{{max}}}}}



\newcommand{\introthresh}{\ensuremath{t}} 


\newcommand{\Uni}{\ensuremath{\operatorname{Uni}}}

\newcommand{\none}{\ensuremath{{\numobs_{1}}}}
\newcommand{\ntwo}{\ensuremath{{\numobs_{2}}}}

\newcommand{\XsamOne}{\ensuremath{\{X_i\}_{i=1}^\none}}
\newcommand{\XsamTwo}{\ensuremath{\{X'_i\}_{i=1}^\ntwo}}

\newcommand{\XbigFullSam}{\ensuremath{{\{X_i\}_{i=1}^{\none + \ntwo}}}}

% Discriminant function
\newcommand{\DiscFun}{\ensuremath{\Psi}}
\newcommand{\DiscFunHat}{\ensuremath{\widehat{\DiscFun}}}
\newcommand{\DiscFunTil}{\ensuremath{\widetilde{\DiscFun}}}
\newcommand{\DiscFunHatSimple}{\ensuremath{\DiscFunHat_{\mathrm{{id}}}}}

%\newcommand{\err}{\ensuremath{\epsilon}}
\newcommand{\err}{\ensuremath{\mbox{Err}}}



% Marcenko-Pastur law
\newcommand{\FMP}{\ensuremath{f_{\mathrm{{MP}}}}}

% Upper and lower limits in Marceko-Pastur law
\newcommand{\tmin}{\ensuremath{t_{\small{\operatorname{min}}}}}
\newcommand{\tmax}{\ensuremath{t_{\small{\operatorname{max}}}}}




\newcommand{\MatCumFunc}[1]{\ensuremath{\Phi_{#1}}}
\newcommand{\MatCumFun}{\MatCumFunc{\Qmat}}

\newcommand{\MatMomFunc}[1]{\ensuremath{\Psi_{#1}}}
\newcommand{\MatMomFun}{\MatMomFunc{\Qmat}}


\newcommand{\bernbou}{\ensuremath{b}}





\newcommand{\Vprime}{\ensuremath{\Vset'}}
\newcommand{\Rcrow}{\ensuremath{R}}



\newcommand{\ksubgauss}{\ensuremath{\sigma}}

\newcommand{\SpecSet}{\ensuremath{\mathbb{K}}}

\newcommand{\SpecSetCov}{\ensuremath{\Sphere{\usedim}(\CovMat^{-1})}}
\newcommand{\CovMatSqrtInv}{\ensuremath{\CovMat^{-\frac{1}{2}}}}
\newcommand{\util}{\ensuremath{\widetilde{u}}}
\newcommand{\uprime}{\ensuremath{u'}}
\newcommand{\vprime}{\ensuremath{v'}}
%\newcommand{\frob}[1]{\ensuremath{\matsnorm{#1}{F}}}
\newcommand{\frob}[1]{\frobnorm{#1}}

\newcommand{\ParSpace}{\ensuremath{\Omega}}
\newcommand{\ParSet}{\ensuremath{\ParSpace}}
\newcommand{\MiniMax}{\ensuremath{\mathfrak{M}}}
\newcommand{\HackMiniMax}{\ensuremath{\MiniMax(\theta(\Pclass),
\MinFun \circ \rhomet)}}

\newcommand{\deltil}{\ensuremath{\widetilde{\delta}}}

%\newcommand{\thetastar}{\ensuremath{\theta^*}}
\newcommand{\Zhat}{\ensuremath{\widehat{Z}}}
\newcommand{\zhat}{\ensuremath{\widehat{z}}}
\newcommand{\Ztil}{\ensuremath{\widetilde{Z}}}
\newcommand{\ztil}{\ensuremath{\widetilde{z}}}


\newcommand{\deln}{\ensuremath{\delta^*}}
\newcommand{\Pbar}{\ensuremath{\widebar{\mathbb{P}}}}
\newcommand{\nullsp}{\ensuremath{\operatorname{null}}}
\newcommand{\Nkull}{\ensuremath{N_{\mathrm{{KL}}}}}

\newcommand{\TermOne}{\ensuremath{\Term_1}}
\newcommand{\TermTwo}{\ensuremath{\Term_2}}
\newcommand{\TermThree}{\ensuremath{\Term_3}}

\newcommand{\NSUM}{\ensuremath{\frac{1}{\numobs} \sum_{i=1}^\numobs}}

\newcommand{\ConeSub}{\ensuremath{\mathbb{C}}}

\newcommand{\perturb}{\ensuremath{\Delta}}
\newcommand{\perturbhat}{\ensuremath{\widehat{\perturb}}}
\newcommand{\Perturb}{\ensuremath{\PertMat}}
\newcommand{\PerturbHat}{\ensuremath{\widehat{\PertMat}}}
\newcommand{\PertHat}{\ensuremath{\widehat{\PertMat}}}
\newcommand{\PertHatPlain}{\ensuremath{\widehat{\Delta}}}

\newcommand{\strongcon}{\ensuremath{\gamma}}
\newcommand{\genparam}{\ensuremath{\theta}}
\newcommand{\genparamstar}{\ensuremath{\genparam^*}}
\newcommand{\genparamhat}{\ensuremath{\widehat{\genparam}}}
\newcommand{\conecon}{\ensuremath{\alpha}}
\newcommand{\ellonerad}{\ensuremath{R_1}}
\newcommand{\nullspace}{\ensuremath{\operatorname{null}}}



\newcommand{\mupar}{\ensuremath{\mu}}
%\newcommand{\jones}{1\!\!1}
\newcommand{\jones}{\mathbb{1}}



\newcommand{\ytil}{\ensuremath{\widetilde{y}}}

\newcommand{\sign}{\ensuremath{\operatorname{sign}}}

\newcommand{\rhopar}{\ensuremath{\rho}}


\newcommand{\mutinco}{\ensuremath{\alpha}}
\newcommand{\cmin}{\ensuremath{c_{\operatorname{min}}}}
\newcommand{\colnorm}{\ensuremath{C}}
%\newcommand{\sign}{\ensuremath{\operatorname{sign}}}
\newcommand{\estim}[1]{\ensuremath{\widehat{#1}}}
%\newcommand{\alhat}{\ensuremath{\widehat{\alpha}}}
%\newcommand{\HyperCube}{\ensuremath{\mathbb{H}}}
\newcommand{\Shat}{\ensuremath{\widehat{S}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\Rmax}{\ensuremath{R_{\tiny{\mbox{max}}}}}

\newcommand{\rmax}{\ensuremath{r_{\max}}}


\newcommand{\metric}{\ensuremath{\rho}}
%\newcommand{\MetSpace}{\ensuremath{\mathbb{X}}}
\newcommand{\MetSpace}{\ensuremath{\Xspace}}

\newcommand{\concfunpl}{\ensuremath{{\large{\alpha}}}}
\newcommand{\concfunal}{\ensuremath{\concfunpl_{\: \mprob}}}
\newcommand{\concfun}{\ensuremath{\concfunpl_{\: {\scriptsize{\mprob, (\MetSpace, \metric)}}}}}
\newcommand{\Enlarge}[2]{\ensuremath{#1^{#2}}}
\newcommand{\PlSet}{\ensuremath{A}}
\newcommand{\phifun}{\ensuremath{\phi}}
\newcommand{\Entpl}{\ensuremath{\Psi}}
\newcommand{\Ent}[1]{\ensuremath{\Entpl_{#1}}}
\newcommand{\MGF}{\ensuremath{\varphi}} 
\newcommand{\xback}[1]{\ensuremath{x_{\backslash #1}}}
\newcommand{\MyXback}[1]{\ensuremath{X_{\backslash #1}}}
\newcommand{\sobfun}{\ensuremath{g}}

\newcommand{\Hemi}[1]{\ensuremath{H_{#1}}}

\newcommand{\tvnorm}[1]{\ensuremath{\| #1\|_{\mathrm{{TV}}}}}

\newcommand{\rprob}{\ensuremath{\mathbb{R}}}

\newcommand{\wass}[2]{\ensuremath{W_{\metric}(#1, \, #2)}}
\newcommand{\wasstwo}[2]{\ensuremath{W_2(#1, \, #2)}}
\newcommand{\wasshamm}[2]{\ensuremath{W_{\mathrm{{Ham}}}(#1, \, #2)}}

\newcommand{\transcost}{\ensuremath{\gamma}}

\newcommand{\SPOT}{\ensuremath{\psi}}

\newcommand{\Htil}{\ensuremath{\widetilde{H}}}

\newcommand{\TayError}{\ensuremath{E}}
\newcommand{\InfConv}{\ensuremath{T}}
\newcommand{\Ltil}{\ensuremath{\widetilde{L}}}
\newcommand{\plwass}{\ensuremath{W_1}}

\newcommand{\Fmax}[1]{\ensuremath{\| #1\|_{\Fclass}}}
\newcommand{\Gmax}[1]{\ensuremath{\| #1\|_{\Gclass}}}
\newcommand{\FmaxShort}{\ensuremath{\Fmax{\EmpDist - \Prob}}}
\newcommand{\GmaxShort}{\ensuremath{\Gmax{\EmpDist - \Prob}}}
\newcommand{\FmaxTwo}[2]{\ensuremath{\| #1\|_{#2}}}

\newcommand{\EmpDist}{\ensuremath{\mprob_\numobs}}

\newcommand{\pProb}{\ensuremath{P}}
\newcommand{\pEmpDist}{\ensuremath{\pProb_\numobs}}

\newcommand{\LossClass}{\ensuremath{\mathfrak{L}}}
\newcommand{\littleloss}{\ensuremath{\mathcal{L}}}
\newcommand{\Rhat}{\ensuremath{\widehat{\Risk}_\numobs}}
\newcommand{\Risk}{\ensuremath{R}}
\newcommand{\SphereSet}{\ensuremath{\mathcal{S}_{\mathrm{{sphere}}}}}

\newcommand{\HalfInt}{\ensuremath{\SetClass_{\mathrm{{left}}}}}
\newcommand{\FullInt}{\ensuremath{\SetClass_{\mathrm{{two}}}}}
\newcommand{\LinClass}{\ensuremath{\mathscr{L}}}

\newcommand{\Zsam}[1]{\ensuremath{Z_{#1}}}
\newcommand{\pdens}{\ensuremath{p}}
\newcommand{\qdens}{\ensuremath{q}}
\newcommand{\udens}{\ensuremath{u}}

\newcommand{\thetaprime}{\ensuremath{\theta_{0}}}
\newcommand{\decrule}{\ensuremath{f}}
\newcommand{\dechat}{\ensuremath{\widehat{\decrule}}}
\newcommand{\decstar}{\ensuremath{\decrule^*}}
\newcommand{\MySet}{\ensuremath{\mathbb{S}}}



\newcommand{\OmegaPrime}{\ensuremath{\Omega_0}}

%\newcommand{\thetastar}{{\ensuremath{\theta^{*}}}}
%\newcommand{\thetatil}{{\ensuremath{\widetilde{\theta}}}}

\newcommand{\AsetRad}{\ensuremath{\mathcal{A}}}


\newcommand{\superrade}[1]{\ensuremath{\rade{1}^{#1}}}
\newcommand{\SAMSUM}{\ensuremath{\sum_{i=1}^\numobs}}
\newcommand{\NORMSAMSUM}{\ensuremath{\frac{1}{\numobs} \SAMSUM}}
\newcommand{\EmpRade}[1]{\ensuremath{\widehat{\mathcal{R}}_\numobs(#1)}}


\newcommand{\fbar}{\ensuremath{\widebar{f}}}
\newcommand{\fbarunder}{\ensuremath{\bar{f}}}
\newcommand{\myhbar}{\ensuremath{\widebar{h}}}
\newcommand{\myhalf}{\ensuremath{\frac{1}{2}}}

\newcommand{\CovHat}{\ensuremath{\widehat{\CovMat}}}

% Notation for generic (random) matrix
%\newcommand{\Gymat}{\ensuremath{{\mathbf{Y}}}}
\newcommand{\Gymat}{\ensuremath{M}}





\newcommand{\ThetaMLE}{\ensuremath{\widehat{\ThetaBf}_{\mathrm{{MLE}}}}}

\newcommand{\usedima}{\ensuremath{{\usedim_1}}}
\newcommand{\usedimb}{\ensuremath{{\usedim_2}}}

\newcommand{\jdima}{\ensuremath{j_1}}
\newcommand{\jdimb}{\ensuremath{j_2}}


\newcommand{\SymPSD}[1]{\ensuremath{\mathcal{S}^{#1 \times #1}_+}}
\newcommand{\SymMat}[1]{\ensuremath{\mathcal{S}^{#1 \times #1}}}

\newcommand{\mytilde}[1]{\ensuremath{\widetilde{#1}}}

\newcommand{\martbsum}{\ensuremath{b}}
\newcommand{\kind}{\ensuremath{k}}
\newcommand{\iind}{\ensuremath{i}}
\newcommand{\jind}{\ensuremath{j}}

\newcommand{\kerind}{\ensuremath{j}}
\newcommand{\pind}{\ensuremath{m}}

\newcommand{\Xdseq}[2]{\ensuremath{X_{#1}^{#2}}}
\newcommand{\MySeq}[2]{\ensuremath{\{#1_{#2}\}_{#2 = 1}^\infty}}
\newcommand{\MySeqZero}[2]{\ensuremath{\{#1_{#2}\}_{#2 = 0}^\infty}}

\newcommand{\DoubSeq}[3]{\ensuremath{\{(#1_{#3}, #2_{#3})\}_{#3 = 1}^\infty}}
\newcommand{\MyTripSeq}[3]{\ensuremath{#1_{#2}^{#3}}}
\newcommand{\subexpvar}{\ensuremath{\nu}}
\newcommand{\Bou}{\ensuremath{B}}
\newcommand{\bou}{\ensuremath{b}}
\newcommand{\BernPar}{\ensuremath{b}}
\newcommand{\Fil}{\ensuremath{\mathcal{F}}}


\newcommand{\SubexpBou}{\ensuremath{\alpha}}
\newcommand{\SubExpNew}{\SubexpNew}
\newcommand{\SubexpNew}{\ensuremath{\SubexpBou}}
\newcommand{\SubexpMin}{\ensuremath{\SubexpNew_*}}
\newcommand{\SubexpMinWide}{\SubexpMin}
\newcommand{\ZurSub}{\ensuremath{\SubexpBou}}
\newcommand{\ZurSubInv}{\ensuremath{\ZurSub^{-1}}}



%\newcommand{\SubexpMin}{\ensuremath{\bar{\SubexpNew}}}
%\newcommand{\SubexpMinWide}{\ensuremath{\widebar{\SubexpNew}}}


\newcommand{\diam}{\ensuremath{\operatorname{diam}}}

\newcommand{\gausspl}{\ensuremath{z}}
\newcommand{\gauss}[1]{\ensuremath{\gausspl_{#1}}}


\newcommand{\GRAYBOX}[1]{\noindent \begin{graybox} \parbox{#1}
\end{graybox}}

\newcommand{\MbernBou}{\ensuremath{b}}
\newcommand{\BernBou}{\ensuremath{M}}
\newcommand{\CumGen}{\ensuremath{\Phi}}

%\newcommand{\sign}{\ensuremath{\operatorname{sign}}}

\newcommand{\Xdomain}{\ensuremath{\mathcal{X}}}

\newcommand{\orpar}{\ensuremath{q}}
\newcommand{\orq}{\ensuremath{\psi_\orpar}}
\newcommand{\ornorm}[1]{\ensuremath{\|#1\|_{\orq}}}
\newcommand{\genpar}{\ensuremath{\theta}}
\newcommand{\genpartwo}{\ensuremath{{\thetatil}}}
\newcommand{\ExsA}{\ensuremath{\Exs_A}}

\newcommand{\CovMatSqrt}{\ensuremath{\sqrt{\CovMat}}}
\newcommand{\vtil}{\ensuremath{\widetilde{v}}}
\newcommand{\plopnorm}[1]{\ensuremath{\matsnorm{#1}{2}}}

\newcommand{\DelMin}{\ensuremath{\Delta_{\operatorname{min}}}}
\newcommand{\DelMax}{\ensuremath{\Delta_{\operatorname{max}}}}
\newcommand{\svmaxbar}{\widebar{\mysingval}_{\operatorname{max}}}
\newcommand{\svminbar}{\widebar{\mysingval}_{\operatorname{min}}}



\newcommand{\iprime}{\ensuremath{{i'}}}
\newcommand{\jprime}{\ensuremath{{j'}}}

\newcommand{\statesp}{\ensuremath{\mathcal{X}}}
\newcommand{\ChainNum}{\ensuremath{L}} 
%\renewcommand{\rhomet}{\ensuremath{d}}
\newcommand{\FunBou}{\ensuremath{B}}
\newcommand{\GenSetTil}{\ensuremath{\widetilde{\GenSet}}}
\newcommand{\SparseSet}{\ensuremath{\mathbb{S}}}
\newcommand{\RankSet}{\ensuremath{\mathbb{M}}}
\newcommand{\fullopnorm}[1]{\ensuremath{\matsnorm{#1}{\ell_2 \rightarrow
      \ell_2}}}


\newcommand{\QmatPol}[1]{\ensuremath{\mathbf{Q}_{#1}}}
\newcommand{\PmatSub}[1]{{\ensuremath{\Pmat_{#1}}}}
\newcommand{\OPOS}{\ensuremath{\mathcal{O}}}
\newcommand{\IdOp}{\ensuremath{\myoperator{I}}}
\newcommand{\Uop}{\ensuremath{\myoperator{U}}}


%\newcommand{\maxnormoff}[1]{\ensuremath{\matsnorm{#1}{\mathrm{{max,off}}}}}
\newcommand{\maxnormoff}[1]{\ensuremath{\|#1\|{\mathrm{{max,off}}}}}

\newcommand{\myvec}{\ensuremath{\operatorname{vec}}}
\newcommand{\MYVEC}[1]{\mathbf{#1}}
\newcommand{\sv}{\ensuremath{\gamma}}

\newcommand{\SetBB}{\ensuremath{\mathbb{T}}}
\newcommand{\NewSetBB}{\ensuremath{\mathbb{U}}}



\newcommand{\istar}{\ensuremath{i^\ast}}



\newcommand{\smallthetahat}{\ensuremath{\hat{\theta}}}

\newcommand{\Uvar}{\ensuremath{U}}

\newcommand{\Xmatt}[1]{\ensuremath{\Xmat_{#1}}}

\newcommand{\subgrad}{\ensuremath{z}}

\newcommand{\taupar}{\ensuremath{\tau}}
\newcommand{\betaplus}{\ensuremath{\beta^+}}
\newcommand{\betaneg}{\ensuremath{\beta^-}}

\newcommand{\bparam}{\ensuremath{\beta}}

\newcommand{\Mnum}{M}
\newcommand{\usen}{\ensuremath{N}}

\newcommand{\basefun}{\ensuremath{\phi}}

\newcommand{\Fclasspara}{\ensuremath{\mathscr{P}}}

\newcommand{\spectheta}{\gamma}
\newcommand{\TrunEllipse}{\ensuremath{\widetilde{\Ellipse}}}
\newcommand{\EllipseTil}{\TrunEllipse}

\newcommand{\jlnum}{\ensuremath{N}}
\newcommand{\jlprojdim}{\ensuremath{m}}
\newcommand{\genthtwo}{\ensuremath{{\widetilde{\gentheta}}}}
%\newcommand{\genthtwo}{\ensuremath{{\gentheta'}}}

\newcommand{\GcovNum}[3]{\ensuremath{N_{#3} \left(#1 \, ; \, #2 \right)}}
\newcommand{\GpackNum}[3]{\ensuremath{M_{#3}(#1 \, ; \, #2)}}
\newcommand{\SetDia}{\ensuremath{D}}
\newcommand{\rehamm}{\ensuremath{\widebar{d}_H}}
\newcommand{\HyperCube}{\ensuremath{\mathbb{H}}}


\newcommand{\Ber}{\ensuremath{\operatorname{Ber}}}
\newcommand{\vsmall}{\vspace*{.1in}}
%\newcommand{\vtiny}{\vspace*{.05in}}


\newcommand{\orpsi}[1]{\ensuremath{\| #1\|_{\psi}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% What to use as the dimension in preliminary work on metric entropy
%\newcommand{\usedim}{\ensuremath{\mdim}} 
\newcommand{\usedim}{\ensuremath{d}} 

\newcommand{\taildim}{n}

\newcommand{\Sigal}{\ensuremath{\mathcal{A}}} 

\newcommand{\mydelta}{\ensuremath{\delta}}
\newcommand{\myeps}{\ensuremath{\epsilon}}


\newcommand{\Mcon}{\ensuremath{\kappa}}
%\newcommand{\NewMcon}{\ensuremath{\Mcon_{\LossSing}}}
%\newcommand{\NewMconBar}{\ensuremath{\widebar{\Mcon}_{\LossSing}}}

\newcommand{\NewMcon}{\ensuremath{\Mcon}}
\newcommand{\NewMconBar}{\ensuremath{\widebar{\Mcon}}}


\newcommand{\ErrRad}{\ensuremath{\TOL}}
\newcommand{\tstar}{\ensuremath{t^\ast}} 


\newcommand{\TOL}{\ensuremath{\delta}}

\newcommand{\Err}[1]{\ensuremath{\|#1\|}}



\newcommand{\Con}{\ensuremath{\eta}}
\newcommand{\KeyCon}[1]{\ensuremath{\Psi(#1)}}
\newcommand{\KeyConSq}[1]{\ensuremath{\Psi^2(#1)}}
\newcommand{\KeyRev}[1]{\ensuremath{\Phi(#1)}}
\newcommand{\KeyConOne}[1]{\ensuremath{\eta_{r;r}(#1)}}
\newcommand{\KeyConDual}[1]{\ensuremath{\eta_{r;e^*}(#1)}}
\newcommand{\KeyConFull}[1]{\ensuremath{\eta(#1; R, e)}}
\newcommand{\KeyConTwo}{\ensuremath{\eta_{r;2}}}
\newcommand{\KeyConTwoReg}{\ensuremath{\eta_{2;r}}}
\newcommand{\KeyConQpar}{\ensuremath{\eta_{(1,\qpar);2}}}


\newcommand{\myrad}{r}
%\newcommand{\KeySet}{\ensuremath{\mathcal{D}}}

\newcommand{\gvar}{\ensuremath{g}}
\newcommand{\gsam}[1]{\ensuremath{\gvar_{#1}}}


\newcommand{\EllInt}{\ensuremath{\mathcal{D}}}
\newcommand{\Ellipse}{\ensuremath{\mathcal{E}}}

\newcommand{\FclassTil}{\ensuremath{\widetilde{\Fclass}}}

\newcommand{\martmax}{\ensuremath{M}}
\newcommand{\martvar}{\ensuremath{C}}

\newcommand{\Mbou}{\ensuremath{M}}
\newcommand{\Ehat}{\ensuremath{\widehat{\mathbb{E}}}}

\newcommand{\Hclass}{\ensuremath{\mathcal{H}}}
\newcommand{\Hfclass}{\ensuremath{\mathscr{H}}}


\newcommand{\Iclass}{\ensuremath{\mathcal{I}}}

\newcommand{\vtiny}{\vspace*{.05in}}

%% Gray color
%\definecolor{MyGray}{rgb}{0.96,0.97,0.98}
\definecolor{MyGray}{rgb}{0.9,0.9,0.9}



\makeatletter\newenvironment{graybox}{ 
\begin{lrbox}{\@tempboxa}
\begin{minipage}{0.985\columnwidth}}{\end{minipage}
\end{lrbox}%
\colorbox{MyGray}{\usebox{\@tempboxa}} }
\makeatother



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter\newenvironment{lemgraybox}{ 
\begin{lrbox}{\@tempboxa}
\begin{minipage}{.98\columnwidth}}{\end{minipage}
\end{lrbox}%
\colorbox{MyGray}{\begin{lemma} \usebox{ \@tempboxa } \end{lemma}} }

\makeatother


%\long\def\greybox#1{%
%    \newbox\contentbox%
%    \newbox\bkgdbox%
%    \setbox\contentbox\hbox to \hsize{%
%        \vtop{
%            \kern\columnsep
%            \hbox to \hsize{%
%                \kern\columnsep%
%                \advance\hsize by -2\columnsep%
%                \setlength{\textwidth}{\hsize}%
%                \vbox{
%                    \parskip=\baselineskip
%                    \parindent=0bp
%                    #1
%                }%
%                \kern\columnsep%
%            }%
%            \kern\columnsep%
%        }%
%    }%
%    \setbox\bkgdbox\vbox{
%        \pdfliteral{0.85 0.85 0.85 rg}
%        \hrule width  \wd\contentbox %
%               height \ht\contentbox %
%               depth  \dp\contentbox
%        \pdfliteral{0 0 0 rg}
%    }%
%    \wd\bkgdbox=0bp%
%    \vbox{\hbox to \hsize{\box\bkgdbox\box\contentbox}}%
%    \vskip\baselineskip%
%}


%\newcommand{\Aclass}{\ensuremath{\mathcal{A}}}


\newcommand{\Dmax}{\ensuremath{D_{\operatorname{max}}}}
\newcommand{\Dmin}{\ensuremath{D_{\operatorname{min}}}}

\newcommand{\edist}{\ensuremath{\stackrel{\mathtiny{d}}{=}}}

\newcommand{\condnum}{\kappa}
\newcommand{\condnumsq}{\kappa^2}

\newcommand{\Xtil}{\ensuremath{\widetilde{X}}}

\newcommand{\Zback}[1]{\ensuremath{Z^{\backslash i}}}





\newcommand{\pseurad}{\ensuremath{D}}
\newcommand{\Dudley}{\ensuremath{\mathcal{J}}}
\newcommand{\setproj}{\ensuremath{\pi}}
\newcommand{\uind}{\ensuremath{u}}

\newcommand{\Qprob}{\ensuremath{\mathbb{Q}}}

\newcommand{\SubClass}{\mathcal{S}} 
\newcommand{\SubGraph}{\ensuremath{S}}

\newcommand{\mathtiny}[1]{\ensuremath{\text{\scriptsize{#1}}}}
\newcommand{\mathsmall}[1]{\ensuremath{\text{\small{#1}}}}

\newcommand{\prevc}{\ensuremath{\vc}}
\newcommand{\vc}{\ensuremath{\nu}}
%\newcommand{\vc}{\ensuremath{d_{\operatorname{{\text{\scriptsize{VC}}}}}}}

\newcommand{\mycard}[1]{\ensuremath{|#1|}}
\newcommand{\plcard}[1]{\ensuremath{\card(#1)}}

\newcommand{\xsamstack}[1]{\ensuremath{x_1^\numobs}}
\newcommand{\Xsamstack}[1]{\ensuremath{X_1^\numobs}}
\newcommand{\Fhat}{\ensuremath{\widehat{F}}}



\newcommand{\Sclass}{\ensuremath{\mathcal{S}}}
\newcommand{\Uclass}{\ensuremath{\mathcal{U}}}

\newcommand{\NatInt}{\ensuremath{\mathbb{N}}}

\newcommand{\SetClass}{\ensuremath{\mathcal{S}}}
\newcommand{\TsetClass}{\ensuremath{\mathcal{T}}}

\newcommand{\htil}{\ensuremath{\widetilde{h}}}
\newcommand{\hstar}{\ensuremath{h^*}}
%\newcommand{\ftil}{\ensuremath{\widetilde{f}}}
\newcommand{\gtil}{\ensuremath{\widetilde{g}}}
\newcommand{\altil}{\ensuremath{\widetilde{\alpha}}}

\newcommand{\newspan}{\ensuremath{\operatorname{span}}}

\newcommand{\Newfclass}{\ensuremath{\mathbb{F}}}
%\newcommand{\Null}{\ensuremath{\mathcal{N}}} 

\newcommand{\zplus}[1]{\ensuremath{(#1)_+}}

\newcommand{\NOTS}{\ensuremath{\backslash \{\ej\}}}

\newcommand{\graph}{\ensuremath{G}}
\newcommand{\graphhat}{\ensuremath{\widehat{\graph}}}
\newcommand{\vertex}{\ensuremath{V}}
\newcommand{\edge}{\ensuremath{E}}
\newcommand{\edgehat}{\ensuremath{\widehat{\edge}}}

\newcommand{\convprob}{\ensuremath{\stackrel{\mathtiny{prob.}}{\longrightarrow}}}
\newcommand{\convas}{\ensuremath{\stackrel{a.s.}{\longrightarrow}}}
\newcommand{\convdist}{\ensuremath{\stackrel{d}{\longrightarrow}}}

\newcommand{\Zfn}{\ensuremath{\Zf_\numobs}}
\newcommand{\Xsamtil}[1]{\ensuremath{\widetilde{X}_{#1}}}
\newcommand{\Xsamprime}[1]{\ensuremath{\Xprime_{#1}}}
\newcommand{\Xback}[1]{\ensuremath{X^{\backslash #1}}}
\newcommand{\funbound}{\ensuremath{b}}
\newcommand{\funbou}{\ensuremath{\funbound}}
\newcommand{\Xprime}{\ensuremath{X'}}
\newcommand{\Ninf}[2]{\ensuremath{N_\infty(#1; #2)}}


\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}



\newcommand{\Radeplain}{\ensuremath{\mathcal{R}}}
\newcommand{\Rade}[1]{\ensuremath{\Radeplain(#1)}}
\newcommand{\Raden}[1]{\ensuremath{\Radeplain_\numobs(#1)}}
\newcommand{\RadeSq}[1]{\ensuremath{\Radeplain^2(#1)}}
\newcommand{\RadenSq}[1]{\ensuremath{\Radeplain_\numobs^2(#1)}}

\newcommand{\noisestd}{\ensuremath{\sigma}}
\newcommand{\noisevar}{\ensuremath{\sigma}}

\newcommand{\pdiff}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand{\kerpsi}{\ensuremath{\psi}}
\newcommand{\gnoisepl}{\ensuremath{g}}
\newcommand{\gnoise}[1]{\ensuremath{\gnoisepl_{#1}}}


\newcommand{\radq}{\ensuremath{R_\qpar}}

\newcommand{\NoiseSeq}{\ensuremath{\{\regnoise{i}\}_{i=1}^\numobs}}

\newcommand{\NonGaussCompSpec}[1]{\ensuremath{\mathcal{G}_{#1}}}

\newcommand{\delcrit}{\ensuremath{\delta_\numobs}}
\newcommand{\delcrithat}{\ensuremath{\hat{\delta}_\numobs}}
\newcommand{\delcritsmallhat}{\ensuremath{\hat{\delta}_\numobs}}

\newcommand{\AUSRIDGE}{8}

\newcommand{\secondnasty}{\ensuremath{128}}
\newcommand{\MyMax}{\ensuremath{Z_\numobs}}
\newcommand{\DeltaHat}{\ensuremath{\hat{\Delta}}}

\newcommand{\NonGaussComp}{\ensuremath{\mathcal{G}_\numobs}}
\newcommand{\NonGaussCompTil}{\ensuremath{\mathcal{\widetilde{G}}_\numobs}}

\newcommand{\plregnoise}{\ensuremath{w}}
\newcommand{\regnoisepl}{\ensuremath{\plregnoise}}
\newcommand{\regnoise}[1]{\ensuremath{\plregnoise_{#1}}}


\newcommand{\NonRad}{\ensuremath{W_\numobs}}


\newcommand{\plxsam}{\ensuremath{x}}
\newcommand{\plysam}{\ensuremath{y}}
\newcommand{\plcapysam}{\ensuremath{Y}}

\newcommand{\EdgeHat}{\ensuremath{\hat{\edge}}}

\newcommand{\EmpRad}{\ensuremath{\LocRad}}
\newcommand{\Data}[1]{\ensuremath{x_1^{#1}}}
\newcommand{\DataCap}[1]{\ensuremath{X_1^{#1}}}
\newcommand{\Zdata}[1]{\ensuremath{Z_1^{#1}}}
\newcommand{\ZdataCap}[1]{\ensuremath{Z_1^{#1}}}

\newcommand{\InterSet}{\ensuremath{\mathbb{S}}}


\newcommand{\nastyplus}{\ensuremath{257}}
\newcommand{\nastycon}{\ensuremath{256}}

\newcommand{\specrad}{\ensuremath{R}}
\newcommand{\wannoy}{\ensuremath{z}}
\newcommand{\Term}{\ensuremath{T}}
\newcommand{\sg}{\ensuremath{\kappa}}

\newcommand{\SamCov}{\ensuremath{\widehat{\CovMat}}}
\newcommand{\SamCovPlain}{\ensuremath{\widehat{\Sigma}}}
\newcommand{\PlainSamCov}{\SamCovPlain}
\newcommand{\SamCovN}{\ensuremath{\SamCov_\numobs}}

\newcommand{\Grat}{\ensuremath{G_\numobs}}



\newcommand{\AuxEvent}{\ensuremath{\mathcal{A}}}

\newcommand{\Ytil}{\ensuremath{\widetilde{Y}}}

\newcommand{\radesq}[1]{\ensuremath{\varepsilon^2(#1)}}
\newcommand{\radepl}{\ensuremath{\varepsilon}}
\newcommand{\rade}[1]{\ensuremath{\radepl_{#1}}}
\newcommand{\LocRad}{\ensuremath{\mathcal{R}_\numobs}}
\newcommand{\LocRadEmp}{\ensuremath{\widehat{\mathcal{R}}_\numobs}}



\newcommand{\epsuse}{\ensuremath{\delta}}
\newcommand{\epscrittil}{\ensuremath{\widetilde{\epsuse}_\numobs}}
\newcommand{\epscrit}{\ensuremath{\epsuse_\numobs}}
\newcommand{\newepscrit}{\ensuremath{\varepsilon_\numobs}}


\newcommand{\felltwo}[1]{\ensuremath{\|#1\|_{L^2(\mprob)}}}
\newcommand{\genfelltwo}[2]{\ensuremath{\|#1\|_{L^2(#2)}}}
\newcommand{\SpecRad}{\ensuremath{R}}


\newcommand{\kerbound}{\ensuremath{\kappa}}

\newcommand{\newrad}{\ensuremath{r}}
\newcommand{\mycon}{\ensuremath{\mu}}


\newcommand{\Event}{\ensuremath{\mathcal{E}}}
\newcommand{\Eventtil}{\ensuremath{\widetilde{\Event}}}

\newcommand{\Tset}{\ensuremath{T}}
\newcommand{\TsetCom}{\ensuremath{{\Tset^c}}}

\newcommand{\Gvar}[1]{\ensuremath{X_{#1}}}
\newcommand{\tind}{\ensuremath{t}}
\newcommand{\sind}{\ensuremath{s}}
\newcommand{\sgstan}[1]{\ensuremath{\sigma(#1)}}
\newcommand{\sgstansq}[1]{\ensuremath{\sigma^2(#1)}}
\newcommand{\pseux}{\ensuremath{\rho_X}}

%\newcommand{\Fclass}{\ensuremath{\mathcal{F}}}
%\newcommand{\Fclass}{\ensuremath{\mathbb{F}}}
\newcommand{\Fclass}{\ensuremath{\mathscr{F}}}
\newcommand{\Gclass}{\ensuremath{\mathscr{G}}}
\newcommand{\Gfclass}{\ensuremath{\mathscr{G}}}
\newcommand{\FclassTwo}{\ensuremath{\Fclass'}}
\newcommand{\FclassBar}{\ensuremath{\widebar{\Fclass}}}
\newcommand{\FclassBarUnder}{\ensuremath{\bar{\Fclass}}}

\newcommand{\Xsam}[1]{\ensuremath{X_{#1}}}

\newcommand{\Zf}{\ensuremath{Z}}


\newcommand{\fancysoln}[1]{
\ifthenelse{\equal{\doctype}{WITHSOLS}}
{
\begin{soln}
#1
\end{soln}
}
{
% Do nothing
}
}


%\newcommand{\mobs}{\ensuremath{\numobs}}

\newcommand{\trace}{\ensuremath{\operatorname{trace}}}
\newcommand{\med}{\ensuremath{\operatorname{med}}}

\newcommand{\Plainrep}{\ensuremath{R}}

\newcommand{\CoverNum}{\ensuremath{N}}

\newcommand{\thetaone}{\ensuremath{\theta}}
\newcommand{\thetatwo}{\ensuremath{\widetilde{\theta}}}

\newcommand{\wtil}{\ensuremath{\widetilde{w}}}

\newcommand{\alphatil}{\ensuremath{\widetilde{\alpha}}}
\newcommand{\ntil}{\ensuremath{\widetilde{\numobs}}}
\newcommand{\tseqtil}[1]{\ensuremath{\widetilde{t}_{#1}}} 
\newcommand{\ftil}{\ensuremath{\widetilde{f}}}



\newcommand{\Nat}{\ensuremath{\mathbb{N}}}

\newcommand{\discent}[1]{\ensuremath{H(#1)}}
\newcommand{\pmasspl}[1]{\ensuremath{p_{#1}}}
\newcommand{\pvec}[1]{\ensuremath{p_{#1}}}

\newcommand{\pvechat}[1]{\ensuremath{\widehat{p}_{#1}}}

\newcommand{\pmass}[2]{\ensuremath{p_{#1}(#2)}}
\newcommand{\qerr}{\ensuremath{q_e}}
\newcommand{\discentcond}[2]{\ensuremath{H(#1 \mid #2)}}
\newcommand{\binent}[1]{\ensuremath{h(#1)}}
\newcommand{\xhat}{\ensuremath{\widehat{X}}}


\newcommand{\kerrank}{\ensuremath{r}}
\newcommand{\betatil}{\ensuremath{\widetilde{\beta}}}
\newcommand{\gammatil}{\ensuremath{\widetilde{\gamma}}}


\newcommand{\qprob}{\ensuremath{\mathbb{Q}}}


\newcommand{\ugenvec}{\ensuremath{u}}
\newcommand{\vgenvec}{\ensuremath{v}}
\newcommand{\wgenvec}{\ensuremath{w}}

\newcommand{\tpt}{\ensuremath{x}}




\newcommand{\MYBIBTIT}{Bibliographic details and background}

% Old form
%\newcommand{\Tspace}{\ensuremath{\mathbb{X}}}
\newcommand{\Tspace}{\ensuremath{\mathcal{X}}}

\newcommand{\Rep}[1]{\ensuremath{\Plainrep_{#1}}}

\newcommand{\xseq}[1]{\ensuremath{x_{#1}}}
\newcommand{\tseq}[1]{\ensuremath{x_{#1}}}
\newcommand{\vseq}[1]{\ensuremath{v_{#1}}}
\newcommand{\useq}[1]{\ensuremath{u_{#1}}}

\newcommand{\VecSpace}{\ensuremath{\mathbb{V}}}

\newcommand{\genin}[3]{\ensuremath{\inprod{#1}{#2}_{#3}}}
\newcommand{\gennorm}[2]{\ensuremath{\|#1\|_{#2}}}


\newcommand{\alphahat}{\alhat}
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
\newcommand{\ppar}{\ensuremath{p}}
\newcommand{\mobs}{\ensuremath{n}}
\newcommand{\Zuni}{\ensuremath{Z}}
\newcommand{\Rad}{\ensuremath{\mathfrak{R}}}
\newcommand{\fstar}{\ensuremath{f^*}}
\newcommand{\gstar}{\ensuremath{{g^*}}}
\newcommand{\radtwo}{\ensuremath{r}}
\newcommand{\polydeg}{\ensuremath{m}}

\newcommand{\goodendex}{\hfill $\clubsuit$}
%\newcommand{\goodendex}{\hfill $\diamondsuit$}
%\newcommand{\goodendex}{\\ $\:$ \hline $\;$ \\}




\long\def\comment#1{}

%% modify cite command to do \cite[e.g, ]{foo1,foo2} 
\makeatletter
\def\@cite#1#2{[\if@tempswa #2 \fi #1]}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\Sam}{\ensuremath{\mathcal{S}}} 

\newcommand{\ysam}[1]{\ensuremath{y_{#1}}}
\newcommand{\xsam}[1]{\ensuremath{x_{#1}}}
\newcommand{\wsam}[1]{\ensuremath{w_{#1}}}


\newcommand{\Ysam}[1]{\ensuremath{Y_{#1}}}


\newcommand{\capysam}[1]{\ensuremath{Y_{#1}}}
\newcommand{\capxsam}[1]{\ensuremath{X_{#1}}}
\newcommand{\capwsam}[1]{\ensuremath{W_{#1}}}




\newcommand{\Hil}{\ensuremath{\mathbb{H}}}


\newcommand{\fhat}{\ensuremath{\widehat{f}}}
\newcommand{\yhat}{\ensuremath{\widehat{y}}}



\newcommand{\Ker}{\ensuremath{\mathcal{K}}}
\newcommand{\Kertwo}[2]{\ensuremath{\Ker(#1, \, #2)}}
\newcommand{\KerTwo}[2]{\ensuremath{\Kertwo{#1}{#2}}}
\newcommand{\KerfunPlain}{\ensuremath{\Ker}}
%\newcommand{\hilin}[2]{\ensuremath{\inprod{#1}{#2}_{\Hil}}}

\newcommand{\alhat}{\ensuremath{\widehat{\alpha}}}

\newcommand{\Kerpl}{\ensuremath{\Kmat}}
\newcommand{\KerplPlain}{\ensuremath{K}}
\newcommand{\KerMat}{\ensuremath{\mathbf{K}}}
\newcommand{\Kerpltil}{\ensuremath{\widetilde{\Kerpl}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\HyperSub}{\ensuremath{\widetilde{\Hyper}}}
\newcommand{\rhohamm}{\ensuremath{\rho_{\scriptsize{H}}}}
\newcommand{\BallHamm}{\ensuremath{\Ball_{\scriptsize{H}}}}

\newcommand{\epspack}{\ensuremath{\epsilon}}

\newcommand{\kaplow}{\ensuremath{\kappa_\ell}}
\newcommand{\betalas}{\ensuremath{\widehat{\beta}^{\scriptsize{LA}}}}

\newcommand{\Interval}{\ensuremath{\mathcal{I}}}

\newcommand{\Hyper}{\ensuremath{\mathcal{H}}}

%\newcommand{\spindex}{\ensuremath{s}}



\newcommand{\tracer}[2]{\ensuremath{\langle \!\langle {#1}, \; {#2}
\rangle \!\rangle}}





\newcommand{\GenSset}{\ensuremath{S}}
\newcommand{\GenTheta}{\ensuremath{\Theta}}

\newcommand{\var}{\ensuremath{\operatorname{var}}}




\newcommand{\CovNum}{\ensuremath{N}}
\newcommand{\PackNum}{\ensuremath{M}}
\newcommand{\PackSet}{\ensuremath{\mathcal{P}}}

\newcommand{\qpar}{\ensuremath{q}}

\newcommand{\pdim}{\ensuremath{p}}





\newcommand{\mprob}{\ensuremath{\mathbb{P}}}
\newcommand{\GenSet}{\ensuremath{\mathbb{T}}}
%\newcommand{\MetSpace}{\ensuremath{\mathbb{X}}}
\newcommand{\rhomet}{\ensuremath{\rho}}
\newcommand{\SuperCovNum}[3]{\ensuremath{\CovNum (#1 \:; \,  #2, \, #3 )}}
\newcommand{\SuperCovLower}[3]{\ensuremath{\CovNum_{#3}(#1 \:; \,  #2)}}
\newcommand{\CovNumTwo}[2]{\ensuremath{\CovNum_2(#1 \:; \,  #2)}}
\newcommand{\PackNumTwo}[2]{\ensuremath{\PackNum_2(#1 \:; \,  #2)}}

\newcommand{\SuperPackNum}[3]{\ensuremath{\PackNum(#1 \:; \,  #2, \, #3)}}
\newcommand{\Ball}{\ensuremath{\mathbb{B}}}
\newcommand{\ddim}{\ensuremath{d}}

\newcommand{\GaussComp}{\ensuremath{\mathcal{G}}}
\newcommand{\GaussCompEmp}{\ensuremath{\mathcal{G}_\numobs}}
\newcommand{\RadComp}{\ensuremath{\mathbf{R}}}

%\newcommand{\MATZERO}{\ensuremath{0}}
\newcommand{\MATZERO}{\ensuremath{\mathbf{0}}}

%\newcommand{\Gvolpl}{\ensuremath{\Gamma_g}}
\newcommand{\Gvolpl}{\ensuremath{\mathcal{G}}}

\newcommand{\RADE}[1]{\ensuremath{\mathcal{R}(#1)}}

\newcommand{\Gvol}[1]{\ensuremath{\Gvolpl(#1)}}
\newcommand{\gentheta}{\ensuremath{\theta}}
\newcommand{\genthetatil}{\ensuremath{{\tilde{\gentheta}}}}

\newcommand{\sgauss}{\ensuremath{w}}
\newcommand{\Sgauss}{\ensuremath{W}}

\newcommand{\rpar}{\ensuremath{p}}


\newcommand{\mdim}{\ensuremath{m}}


\newcommand{\mymathbf}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\Ymat}{\ensuremath{\mymathbf{Y}}}
\newcommand{\Dmat}{\ensuremath{\mymathbf{D}}}
\newcommand{\Zmat}{\ensuremath{\mymathbf{Z}}}
\newcommand{\Zmatsub}[1]{\ensuremath{\mymathbf{Z}}_{#1}}
\newcommand{\ZhatMat}{\ensuremath{\widehat{\Zmat}}}
\newcommand{\ZtilMat}{\ensuremath{\mymathbf{\Ztil}}}
\newcommand{\XtilMat}{\ensuremath{\widetilde{\Xmat}}}
\newcommand{\XmatTil}{\XtilMat}
\newcommand{\Mmat}{\ensuremath{\mymathbf{M}}}
\newcommand{\Nmat}{\ensuremath{\mymathbf{N}}}
\newcommand{\Smat}{\ensuremath{\mymathbf{S}}}
\newcommand{\Wmat}{\ensuremath{\mymathbf{W}}}
\newcommand{\Hmat}{\ensuremath{\mymathbf{H}}}
\newcommand{\Amat}{\ensuremath{\mymathbf{A}}}
\newcommand{\Tmat}{\ensuremath{\mymathbf{T}}}
\newcommand{\Lmat}{\ensuremath{\mymathbf{L}}}
\newcommand{\Qmat}{\ensuremath{\mymathbf{Q}}}
\newcommand{\Kmat}{\ensuremath{\mymathbf{K}}}
\newcommand{\Rmat}{\ensuremath{\mymathbf{R}}}
\newcommand{\Pmat}{\ensuremath{\mymathbf{P}}}
\newcommand{\Bmat}{\ensuremath{\mymathbf{B}}}
\newcommand{\Vmat}{\ensuremath{\mymathbf{V}}}
\newcommand{\Umat}{\ensuremath{\mymathbf{U}}}
\newcommand{\UmatHat}{\ensuremath{\widehat{\Umat}}}
\newcommand{\Cmat}{\ensuremath{\mymathbf{C}}}
\newcommand{\Emat}{\ensuremath{\mymathbf{E}}}
\newcommand{\MatVar}{\ensuremath{\mymathbf{V}}}

\newcommand{\ZeroMat}{\mathbf{0}}

%\newcommand{\Qmat}{\ensuremath{Q}}


\newcommand{\svarb}[1]{\ensuremath{\mysingval_{#1}}}
\newcommand{\svarbsq}[1]{\ensuremath{\mysingval^2_{#1}}}
\newcommand{\svarbfour}[1]{\ensuremath{\mysingval^4_{#1}}}
\newcommand{\svmax}{\ensuremath{\mysingval_{\operatorname{max}}}}
\newcommand{\svmin}{\ensuremath{\mysingval_{\operatorname{min}}}}
%\newcommand{\mprob}{\ensuremath{\mathbb{P}}}

\newcommand{\regx}{\ensuremath{x}}
\newcommand{\regw}{\ensuremath{w}}
\newcommand{\regy}{\ensuremath{y}}

\newcommand{\PlainSphere}{\ensuremath{\mathbb{S}}}
\newcommand{\Sphere}[1]{\ensuremath{\PlainSphere^{#1-1}}}
\newcommand{\SphereClose}[1]{\ensuremath{\widebar{\PlainSphere}^{#1-1}}}

\newcommand{\gencon}{\ensuremath{c}}

\newcommand{\uone}{\ensuremath{u}} 
\newcommand{\vone}{\ensuremath{v}}
\newcommand{\utwo}{\ensuremath{\tilde{\uone}}}
\newcommand{\vtwo}{\ensuremath{\tilde{\vone}}}

\newcommand{\SuperSet}{\ensuremath{T}}

%\newcommand{\vup}[1]{\ensuremath{v_{#1}}}
%\newcommand{\uup}[1]{\ensuremath{u_{#1}}}

\newcommand{\vup}[1]{\ensuremath{v^{#1}}}
\newcommand{\uup}[1]{\ensuremath{u^{#1}}}


\newcommand{\ballrad}{\ensuremath{r}}



\newcommand{\ysca}{\ensuremath{y}}
\newcommand{\wsca}{\ensuremath{w}}



\newcommand{\xrow}{\ensuremath{x}}
\newcommand{\betastar}{\ensuremath{\beta^*}}


\newcommand{\betahat}{{\ensuremath{{\widehat{\beta}}}}}

\newcommand{\betals}{\ensuremath{\widehat{\beta}^{\;\mathtiny{LS}}}}
\newcommand{\rid}{\operatorname{\mathtiny{RG}}}
\newcommand{\betarid}{\ensuremath{\widehat{\beta}^{\; \rid}}}
\newcommand{\frid}{\ensuremath{f^{\rid}}}


\newcommand{\Loss}{\ensuremath{\LossSing_\numobs}}
\newcommand{\LossSing}{\ensuremath{\mathcal{L}}}
\newcommand{\LossBar}{\ensuremath{\widebar{\LossSing}}}
\newcommand{\LossSingBar}{\ensuremath{\widebar{\LossSing}}}

%\newcommand{\delLike}{\ensuremath{\delta \LossSing_{\tparam}}}
%\newcommand{\delLikeBar}{\ensuremath{\delta \LossSingBar_{\tparam}}}

\newcommand{\delLikeSing}{\ensuremath{\mathcal{E}}}
\newcommand{\delLike}{\ensuremath{\delLikeSing_\numobs}}
\newcommand{\delLikeBar}{\ensuremath{\mathcal{\widebar{E}}}}



\newcommand{\regpar}{\ensuremath{\lambda}}

\newcommand{\CovMat}{\ensuremath{\mathbf{\Sigma}}}
\newcommand{\CovMatPlain}{\ensuremath{\Sigma}}

\newcommand{\ThetaBf}{\ensuremath{\mathbf{\Theta}}}
\newcommand{\ThetaBfTil}{\ensuremath{\widetilde{\ThetaBf}}}

\newcommand{\CovMatStar}{\ensuremath{\CovMat^*}}

\newcommand{\plaincon}{\ensuremath{c}}

\newcommand{\lammin}{\ensuremath{\myeigval_{\operatorname{\scriptsize{min}}}}}
\newcommand{\lammax}{\ensuremath{\myeigval_{\operatorname{\scriptsize{max}}}}}

\newcommand{\mybetaup}[1]{\ensuremath{\beta^{#1}}}
\newcommand{\BetaSet}{\ensuremath{\Theta}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}


% NEW MJW VERSION

% COMPUTER MODERN
%\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
%\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}


% MATHTIMES

%\newcommand{\matnorm}[3]{| || #1 |||_{{#2}, {#3}}}


\newcommand{\mns}{\mkern-1mu}  % My negative space






\newcommand{\covv}[3]{\ensuremath{\cov_{#3}\{#1, \, #2\}}}


%\newcommand{\kull}[2]{\ensuremath{D(#1\; \| \; #2)}}

% IEEE Trans. Info. Theory form of Kullback-Leibler
\newcommand{\kullinf}[2]{\ensuremath{D(#1\, \| \, #2)}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Noise vector
\newcommand{\wvec}{\ensuremath{w}}
\newcommand{\Wvec}{\ensuremath{W}}

% Error vector
\newcommand{\evec}{\ensuremath{e}}

\newcommand{\Exs}{\ensuremath{\mathbb{E}}}




==> Plots/Plots_repoduce_and_data_reproduce_readme.tex <==
# The codes for generating the data are in the folders where the data is stored. 

This is a readme file for generating all the plots used in the paper from already saved data. 


The plot codes for generating plots are in the folder Plots/code_for_generating_plots

==> commands-cleaned-arXiv.tex <==
%!TEX root = instance-value-function-paper.tex

\usepackage{comment}
\usepackage{epsf}
%\usepackage{fancyheadings}
%\usepackage{graphics}
\usepackage{graphicx}

\usepackage{subfigure}
%\usepackage{subcaption}
%\usepackage{psfrag}

\usepackage{color}

\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath, bm}
\usepackage{amssymb}

\usepackage{pgfplots}
\pgfplotsset{width=5.35cm,compat=1.9}

%\usepackage{pgfplots}
%\pgfplotsset{width=6.45cm,compat=1.9}

\usepackage{textcomp}
\usepackage{xcolor}


%\usepackage{fdsymbol}
%\usepackage[linesnumbered, ruled, vlined]{algorithm2e}
%\usepackage{ntheorem}
\usepackage[ruled, vlined, lined, commentsnumbered]{algorithm2e}
%\usepackage[backend=bibtex,firstinits=true]{biblatex}

%\setlength{\textwidth}{\paperwidth}
%\addtolength{\textwidth}{-6cm}
%\setlength{\textheight}{\paperheight}
%\addtolength{\textheight}{-4cm}
%\addtolength{\textheight}{-1.1\headheight}
%\addtolength{\textheight}{-\headsep}
%\addtolength{\textheight}{-\footskip}
%\setlength{\oddsidemargin}{0.5cm}
%\setlength{\evensidemargin}{0.5cm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS HERE

%%%%%%%
%\theoremstyle{plain}

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper

%\theoremprework{\begin{minipage}{\textwidth}}
%\theorempostwork{\end{minipage}}

\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}



%%%%%%%%%%%
%Biber

\usepackage[maxalphanames=4, maxcitenames=3, minalphanames=3, minnames=1, maxnames=50, style=alphabetic, backend=biber, firstinits=true, url=true]{biblatex}\addbibresource{MRPs.bib}
%\usepackage[maxalphanames=4, maxcitenames=3, minalphanames=3, minnames=1, maxnames=50, style=alphabetic, backend=biber, firstinits=true, url=true]{biblatex}\addbibresource{max-aff.bib}
%\renewbibmacro{in:}{}
%% BEGIN HACK: for alpha style bibliography with biblatex
%\renewcommand*{\labelalphaothers}{}
%\DeclareLabelalphaTemplate{
%\labelelement{
%\field[final]{shorthand}
%\field{label}
%\field[strwidth=3,strside=left]{labelname}
%}
%\labelelement{
%\field[strwidth=2,strside=right]{year}
%}
%}


%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
%\newlength{\widebarargwidth}
%\newlength{\widebarargheight}
%\newlength{\widebarargdepth}
%\DeclareRobustCommand{\widebar}[1]{%
%  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
%  \settoheight{\widebarargheight}{\ensuremath{#1}}%
%  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
%  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
%  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
%  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
%    \hspace{0.3\widebarargdepth}%
%    \addtolength{\widebarargheight}{0.3ex}%
%    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
%  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
%\makeatletter
%\long\def\@makecaption#1#2{
%        \vskip 0.8ex
%        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
%        \parindent 1.5em  %% How can we use the global value of this???
%        \dimen0=\hsize
%        \advance\dimen0 by -3em
%        \ifdim \wd\@tempboxa >\dimen0
%                \hbox to \hsize{
%                        \parindent 0em
%                        \hfil 
%                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
%                                {\bf #1.} #2
%                                %%\unhbox\@tempboxa
%                                } 
%                        \hfil}
%        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
%        \fi
%        }
%\makeatother



%% COMMENTING commands

\long\def\comment#1{}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\mjwcomment}[1]{{\bf{{\red{{MJW --- #1}}}}}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\apcomment}[1]{{\bf{{\blue{{AP --- #1}}}}}}



% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

\newcommand{\defn}{:\,=}

\DeclareMathOperator*{\minimize}{minimize}
% Indpendence symbol
\newcommand\indpt{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\sgn}{\mathsf{sgn}}
\newcommand{\conv}{\mathsf{conv}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\polylog}{\mathsf{polylog}}

\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{F}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}
\newcommand{\norms}[1]{\left\|#1 \right\|}

\newcommand{\paren}[1]{\left\{ #1 \right\} }

\newcommand{\eucnorm}[1]{\left\|#1 \right\|}
\newcommand{\linfnorm}[1]{\left\|#1 \right\|_\infty}

\newcommand{\abs}[1]{\ensuremath{ \left| #1 \right|}}

\newcommand{\angles}[2]{\angle  #1 , #2 }
\newcommand{\minangle}[1]{\ensuremath{\alpha_{#1}}}
\newcommand{\sig}[1]{\ensuremath{\theta^{(#1)}}}
\newcommand{\appsig}[1]{\ensuremath{\beta^{(#1)}}}
\newcommand{\sigloo}[2]{\ensuremath{\theta^{(#1)}_{\backslash #2}}}
\newcommand{\sigtil}[2]{\ensuremath{\thetatil^{(#1)}_{#2}}}

\newcommand{\vstar}{\ensuremath{v^*}}
\newcommand{\ustar}{\ensuremath{u^*}}
\newcommand{\wstar}{\ensuremath{w^*}}
\newcommand{\vvec}[1]{\ensuremath{v^{(#1)}}}
\newcommand{\del}[1]{\ensuremath{\Delta^{(#1)}}}
\newcommand{\uvec}[1]{\ensuremath{u^{(#1)}}}
\newcommand{\Deltamax}{\ensuremath{\mathsf{B}_{\mathsf{max}}}}

\newcommand{\Sup}[1]{\ensuremath{\mathsf{S}^{(#1)}}}
\newcommand{\sball}{\ensuremath{\zeta}}
\newcommand{\pimin}{\ensuremath{\pi_{\min}}}
\newcommand{\cs}{\ensuremath{c_{\mathsf{s}}}}
\newcommand{\Csig}{\ensuremath{C_{\eta, \sball, \cs}}}

\newcommand{\msdiff}{\ensuremath{\varrho}}

\newcommand{\Bvol}{\ensuremath{\mathtt{B}_{\mathsf{vol}}}}

\newcommand{\Sset}[1]{\ensuremath{\mathsf{S}_{#1}}}
\newcommand{\Scomp}[1]{\ensuremath{\mathsf{S}^c_{#1}}}
% Observations, dimension etc.
\newcommand{\numdim}{\ensuremath{d}}
\newcommand{\numobs}{\ensuremath{n}}

\DeclareMathOperator{\tr}{{\sf tr}}
\newcommand{\ones}{\ensuremath{{\bf 1}}}

% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

% Kullback-Leibler
\newcommand{\kull}[2]{\ensuremath{D_{\mathsf{KL}}(#1\; \| \; #2)}}
\newcommand{\KL}{\ensuremath{D_{\mathsf{KL}}}}
\newcommand{\TV}{\ensuremath{D_{\mathsf{TV}}}}

% Probability
\newcommand{\E}{\ensuremath{{\mathbb{E}}}}
\newcommand{\EE}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}

\newcommand{\ind}[1]{\ensuremath{{\mathbf{1}\left\{ #1 \right\}}}}




%Numbering
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
\newcommand{\6}{\ensuremath{{\sf (vi)}}}

%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}

\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\floor}{floor}
\DeclareMathOperator{\vol}{\mathfrak{vol}}
\DeclareMathOperator{\rank}{{\sf rank}}
\DeclareMathOperator{\card}{{\sf card}}
\DeclareMathOperator{\range}{{\sf range}}


% Distributions
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{\sf Ber}}}
\newcommand{\BIN}{\ensuremath{\mbox{\sf Bin}}}
\newcommand{\Hyp}{\ensuremath{\mbox{\sf Hyp}}}
\newcommand{\Pdist}{\ensuremath{\mathbb{P}}}
\newcommand{\Qdist}{\ensuremath{\mathbb{Q}}}

% Script letters
\newcommand{\Aspace}{\ensuremath{\mathcal{A}}}
\newcommand{\Dspace}{\ensuremath{\mathcal{D}}}
\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}
\newcommand{\Espace}{\ensuremath{\mathcal{E}}}
\newcommand{\Ispace}{\ensuremath{\mathcal{I}}}
\newcommand{\Mspace}{\ensuremath{\mathfrak{M}}}
\newcommand{\Uspace}{\ensuremath{\mathcal{U}}}
\newcommand{\Sspace}{\ensuremath{\mathcal{S}}}
\newcommand{\Rspace}{\ensuremath{\mathcal{R}}}
\newcommand{\Wspace}{\ensuremath{\mathcal{W}}}
\newcommand{\Cspace}{\ensuremath{\mathcal{C}}}
\newcommand{\Bspace}{\ensuremath{\mathcal{B}}}
\newcommand{\Pspace}{\ensuremath{\mathcal{P}}}
\newcommand{\Lspace}{\ensuremath{\mathcal{L}}}
\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\lossn}[1]{\ensuremath{\mathcal{L}^n \left( #1 \right)}}
% Basic statistics notation
% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
% Estimates
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
\newcommand{\Mhat}{\ensuremath{\widehat{M}}}
\newcommand{\bhat}{\ensuremath{\widehat{b}}}
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}

\newcommand{\Ttil}{\ensuremath{\widetilde{\T}}}
\newcommand{\That}{\ensuremath{\widehat{\T}}}
\newcommand{\T}{\ensuremath{\mathcal{T}}}

\newcommand{\etatil}{\ensuremath{\widetilde{\eta}}}

\newcommand{\xitil}{\ensuremath{\widetilde{\xi}}}
\newcommand{\tautil}{\ensuremath{\widetilde{\tau}}}
\newcommand{\mutil}{\ensuremath{\mu_{\tau}}}
\newcommand{\Sigmatil}{\ensuremath{\Sigma_{\tau}}}

\newcommand{\thetarr}{\ensuremath{\widehat{\theta}_{{\sf RR}}}}
\newcommand{\thetahatts}{\ensuremath{\widehat{\theta}_{\mathsf{TS}}}}
%\newcommand{\thetahatls}{\ensuremath{\widehat{\theta}_{\mathsf{LS}}}}
\newcommand{\thetahatsp}{\ensuremath{\widehat{\theta}_{\mathsf{SP}}}}
\newcommand{\ahatls}{\ensuremath{\widehat{A}_{\mathsf{LS}}}}
\newcommand{\Thetastar}{\ensuremath{\Theta^*}}
\newcommand{\Thetahat}{\ensuremath{\widehat{\Theta}}}
\newcommand{\Thetahatls}{\ensuremath{\widehat{\Theta}_{\mathsf{LS}}}}

\newcommand{\thetahatls}{\ensuremath{\widehat{\theta}^{\mathsf{LS}}}}
\newcommand{\thetahatam}{\ensuremath{\widehat{\theta}^{\mathsf{AM}}}}
\newcommand{\bhatls}{\ensuremath{\widehat{b}^{\mathsf{LS}}}}
\newcommand{\bhatam}{\ensuremath{\widehat{b}^{\mathsf{AM}}}}

% Order notation
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\ordertil}{\ensuremath{\widetilde{\order}}}
\newcommand{\Omegatil}{\ensuremath{\widetilde{\Omega}}}

\newcommand{\yvec}{\ensuremath{y}}
\newcommand{\Xmat}{\ensuremath{X}}
\newcommand{\AppXmat}{\ensuremath{\Xi}}
\newcommand{\sigstar}{\ensuremath{\theta^*}}
\newcommand{\bstar}{\ensuremath{b^*}}
\newcommand{\appsigstar}{\ensuremath{\beta^*}}
\newcommand{\vstarone}{\ensuremath{v^*_1}}
\newcommand{\vstartwo}{\ensuremath{v^*_2}}
\newcommand{\xistar}{\ensuremath{\xi^*}}
\newcommand{\meas}{\ensuremath{x}}
\newcommand{\appmeas}{\ensuremath{\xi}}
\newcommand{\obs}[2]{\ensuremath{ \inprod{\meas_{#1}}{\sig{#2}}}}
\newcommand{\obsstar}[1]{\ensuremath{ \inprod{\meas_{#1}}{\sigstar}}}

\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\Sd}{\ensuremath{\mathbb{S}^{d-1}}}
\newcommand{\Bd}{\ensuremath{\mathbb{B}^{d}}}

\newcommand{\Uhat}{\ensuremath{\widehat{U}}}
%\newcommand{\Vhat}{\ensuremath{\widehat{V}}}
\newcommand{\Vstar}{\ensuremath{V^*}}
\newcommand{\Ustar}{\ensuremath{U^*}}
\newcommand{\Astar}{\ensuremath{A^*}}

\newcommand{\ellsharp}{\ensuremath{\ell^{\#}}}
%\newcommand{\Thetahatls}{\ensuremath{\widehat{\Theta}_{\mathsf{LS}}}}
\newcommand{\st}{\ensuremath{\; \Big | \;}}

% Notation for RL/Q-learning

\newcommand{\Qval}[1]{\ensuremath{Q^{#1}}}
\newcommand{\Qhat}[1]{\ensuremath{\widehat{Q}^{#1}}}
\newcommand{\Vval}[1]{\ensuremath{V^{#1}}}
\newcommand{\Vhat}[1]{\ensuremath{\widehat{V}^{#1}}}

\newcommand{\ValueFunc}{\ensuremath{\theta}}
\newcommand{\ValueFunchat}{\ensuremath{\widehat{\theta}_{\mathsf{plug}}}}
\newcommand{\ValueFunchatrob}{\ensuremath{\widehat{\theta}_{\mathsf{MoM}}}}

\newcommand{\Belpop}{\ensuremath{\mathcal{T}}}
\newcommand{\Belemp}{\ensuremath{\widehat{\mathcal{T}}}}

\newcommand{\MoM}{\ensuremath{\widehat{\mathcal{M}}}}
\newcommand{\muhat}{\ensuremath{\widehat{\mu}}}

\newcommand{\robust}{\ensuremath{\mathsf{MoM}}}
\newcommand{\plugin}{\ensuremath{\mathsf{plug}}}

\newcommand{\Belplugin}{\ensuremath{\widetilde{\mathcal{T}}}}

\newcommand{\rdist}{\ensuremath{\mathcal{D}_r}}
\newcommand{\sigmar}{\ensuremath{\sigma(\rstar)}}

\newcommand{\Nsamp}{\ensuremath{N}}
\newcommand{\Dim}{\ensuremath{D}}

\newcommand{\phat}{\ensuremath{\widehat{p}}}
\newcommand{\PmatTil}{\ensuremath{\widetilde{\Pmat}}}

\newcommand{\DelHatIpert}{\ensuremath{\DelHat^{(i)}}}
\newcommand{\thetahatIpert}{\ensuremath{\thetahat^{(i)}}}
\newcommand{\pmat}{\ensuremath{p}}
\newcommand{\Phatloo}[1]{\Phat^{(#1)}}
\newcommand{\Mhatloo}[1]{\MoM^{(#1)}}

\newcommand{\basic}{\mathbf{0}}

%\newcommand{\var}{\mathsf{var}}
\newcommand{\val}{\mathsf{vfun}}
\newcommand{\rew}{\mathsf{rew}}
\newcommand{\Zmattil}{\widetilde{\mathbf{Z}}}

%Upper bounds on the various problem-dependent qtys
\newcommand{\sigvalbd}{\ensuremath{\vartheta}}
\newcommand{\sigrewbd}{\ensuremath{\varrho}}
\newcommand{\valbd}{\ensuremath{\zeta}}

\newcommand{\lbmaxrew}{\ensuremath{\nu}}
\newcommand{\rewfourthstate}{\ensuremath{\phi}}
